CANDY: A Benchmark for Continuous Approximate Nearest Neighbor Search with Dynamic Data Ingestion

Approximate K Nearest Neighbor (AKNN) algorithms play a pivotal role in various AI applications, including information retrieval, computer vision, and natural language processing. Although numerous AKNN algorithms and benchmarks have been developed recently to evaluate their effectiveness, the dynamic nature of real-world data presents significant challenges that existing benchmarks fail to address. Traditional benchmarks primarily assess retrieval effectiveness in static contexts and often overlook update efficiency, which is crucial for handling continuous data ingestion. This limitation results in an incomplete assessment of an AKNN algorithms ability to adapt to changing data patterns, thereby restricting insights into their performance in dynamic environments. To address these gaps, we introduce CANDY, a benchmark tailored for Continuous Approximate Nearest Neighbor Search with Dynamic Data Ingestion. CANDY comprehensively assesses a wide range of AKNN algorithms, integrating advanced optimizations such as machine learning-driven inference to supplant traditional heuristic scans, and improved distance computation methods to reduce computational overhead. Our extensive evaluations across diverse datasets demonstrate that simpler AKNN baselines often surpass more complex alternatives in terms of recall and latency. These findings challenge established beliefs about the necessity of algorithmic complexity for high performance. Furthermore, our results underscore existing challenges and illuminate future research opportunities. We have made the datasets and implementation methods available at: https://github.com/intellistream/candy.

==> Background.tex <==
\section{Background and Related Work}
\label{sec:bg}
This section discusses xxx. More related work discussions are presented in Appendix~\ref{appendix:related}.

\textbf{AKNN concepts.}
Nearest Neighbor Search is a fundamental operation in the data science community~\cite{}. Specifically, given a query \queryCommand, nearest neighbor search aims at searching \annk \emph{closest} vectors among all of the ingested vectors, denoted as \vectorSet. There are various distance measures to define the ``closest'', and two common measures are L2 distance~\cite{li2019approximate} and Inner Product Distance~\cite{aguerrebere2024locally}. Intuitively, this requires exhaustive traversal over \vectorSet to compute distance and compare the vectors, and such an exact but brutal force approach is selected as the baseline (denoted as \algoBF for short) in the following.

AKNN aims to avoid exhaustive traversal over \vectorSet by using approximate computing. Specifically, it selects a subset from \vectorSet, denoted as \vectorSubset (i.e., $\vectorSubsetInEq \subseteq \vectorSetInEq$). 
By \vectorSubset-based searching instead of a full scan of \vectorSet, AKNN is considered to achieve superior retrieval efficiency than \algoBF.
%
The result of AKNN is represented by \resulSetAKNN, which contains \annk vectors from the subset \vectorSubset.
%
The set \resulSetAKNN typically differs from the exact search result \resulSet, and the disparity between \resulSetAKNN and \resulSet serves as the accuracy metric for AKNN, often referred to as ``recall'' and denoted as \recall. Specifically, \recall is a fractional value calculated as $\recallInEq = \frac{|\resulSetAKNNInEq \cap \resulSetInEq|}{\annkInEq}$.

\begin{table}[]
\centering
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{|c|l|l|}
\hline
\multicolumn{1}{|c|}{\textit{Category}} & \textit{Algorithm Name}                & \textit{Descriptions}                                                                                             \\ \hline
\multirow{7}{*}{Ranging-based}        
& \algoLSH~\cite{gionis1999similarity}   & Data-independednt hashing to determine ranges                                                                     \\ \cline{2-3} 
                                        & \algoPQ~\cite{jegou2010product}        & Product quantization to determin ranges                                                                           \\ \cline{2-3} 
                                        & \algoIVFPQ~\cite{jegou2010product}     & Hierachical optimization over \algoPQ                                                                             \\ \cline{2-3} 
                                        & \algoFlann~\cite{muja2014scalable}     & Space partition to determine ranges                                                                               \\ \cline{2-3} 
                                        & \algoBatl~\cite{li2023learning}        & Machine learning to determine ranges  \\ \cline{2-3}   & \algoOnlinePQ~\cite{xu2018online}        & Incrementally update centroids of \algoPQ 
                                                                                  \\ \hline
\multirow{5}{*}{Navigation-based}       & \algoNSW~\cite{malkov2014approximate}  & Delaunay Graph for navigation                                                                                     \\ \cline{2-3} 
                                        & \algoNNDecent~\cite{dong2011efficient} & K-Nearest Neighbor Graph for navigation                                                                           \\ \cline{2-3} 
                                        & \algoDPG~\cite{li2019approximate}      & \begin{tabular}[c]{@{}l@{}}K-Nearest Neighbor Graph and Relative Neighborhood Graph\\ for Navigation\end{tabular} \\ \cline{2-3} 
                                        & \algoNSG~\cite{fu2019fast}      & \begin{tabular}[c]{@{}l@{}} Optimized vertex assignment compared with \algoDPG \end{tabular} \\ \cline{2-3} 
                                        & \algoHNSW~\cite{malkov2018efficient}   & Hiearchical construction of \algoNSW                                                                                                                                                       \\ \hline
\end{tabular}
}
\caption{Studied AKNN algorithms}
\label{tab:algosList}
\end{table}

Depending on the major difference of how \vectorSubset is generated, 
we broadly classify the state-of-the-art ANNS algorithms into two
main categories in the following: ranging-based and navigation-based, as summarized in Table~\ref{tab:algosList}. 
%We discuss the existing comparison results of these categories at the end of this section.


%This paper proposes the first comprehensive benchmark study to revisit vector indexing under online ingestion. It evaluates numerous vector indexing algorithms, with a focus on those allowing or specifically designed for online updates. Our study encompasses various datasets and updating patterns. 
\textbf{Ranging-based AKNN.} Ranging-based AKNN utilizes pre-computed range division of \vectorSet regardless of the specific \queryCommand.
Specifically, it firstly divides \vectorSet into disjoint ranges $D_1, D_2,...,D_n$. When encountering a \queryCommand, the \vectorSubset is directly picked by using a pre-computed range (e.g., $\vectorSubsetInEq = D_1$), or using the union of several ranges (e.g., $\vectorSubsetInEq = D_1 \cup D_2$). 

Locality Sensitive Hashing (\algoLSH~\cite{gionis1999similarity} is perhaps the first ranging-based AKNN and also the first version of AKNN. It tries to hash similar vectors into the same bucket and distant vectors into different buckets by probability, and each bucket forms a range $D_i$.
%
\algoLSH is usually criticized for the suboptimal tradeoff between retrieving efficiency and recall \recall. 
%
 To get a better organization of ranges and make similar vectors more likely to be located in the same range, 
The follow-up ranging-based AKNN explores replacing the hashing function with more sophisticated approaches.
%
This is typically achieved by considering the distribution of \vectorSet, such as product quantization (\algoPQ~\cite{jegou2010product}) and space partition (\algoFlann~\cite{muja2014scalable}). 
%
The hierarchical layout of the ranges is also introduced to further enhance the retrieving efficiency, such as \algoIVFPQ~\cite{jegou2010product} which utilizes two tiers of quantizers to further improve \algoPQ.
%


%such as \algoBatl~\cite{li2023learning}, which utilizes a deep neural network composed of Transformers and Multilayer Perceptron to learn an optimal hierarchical space partition to determine the ranges.
%

\xianzhi{Ranging-based AKNN entails a simple workflow for both data retrieval and ingestion. However, a prevalent challenge is the imperfect determination of ranges in practice. This can result in assigning distant vectors to the same range or assigning similar vectors to distant ranges. Moreover, most ranging-based AKNN methods rely on the further assumption that the distribution of \vectorSet is known and remains constant. 
A well-known exception is \algoOnlinePQ, which improves the \algoPQ by incrementally updating its cluster centroids~\cite{xu2018online}. Ideally, \algoOnlinePQ is able to get updated with the shifted distributions of newly ingested data.
%However, as we will demonstrate in Section~\ref{subsec:overall}, this is still far from realistic real-world action, leading to either reduced recall (\recall) or imposing a substantial penalty of re-assigning ranges.
}

\textbf{Navigation-based AKNN.} 
The navigation-based AKNN method establishes a navigational connection to associate each ingested vector in the data collection \vectorSet with its similar vectors, often achieved by using a proximity graph.
%
In contrast to employing pre-computed ranges, the chosen subset (\vectorSubset) is constructed anew for every query (\queryCommand) by iteratively adding candidate vectors during the navigation process from one vector to its neighboring vectors.
%

The primary distinction among various navigation-based AKNN approaches lies in their diverse strategies for determining the navigation path and deciding when to terminate the expansion of candidate neighbors.
%
For example, \algoNSW~\cite{malkov2014approximate} employs the Delaunay Graph strategy, while \algoNNDecent~\cite{dong2011efficient} utilizes the K-Nearest Neighbor Graph strategy. \algoDPG~\cite{li2019approximate} and \algoNSG~\cite{fu2019fast} share a similar overall design, strategically leveraging the K-Nearest Neighbor Graph and Relative Neighborhood Graph approach. However, \algoNSG proposes to improve the retrieval efficiency of \algoDPG by using different implementations of assigning graph vertices.
%
Additionally, hierarchical design is evident in navigation-based AKNN, reminiscent of ranging-based AKNN. Notably, \algoHNSW~\cite{malkov2018efficient} constructs layers of \algoNSW instead of a flat structure, thereby enhancing retrieval efficiency.
%
The recent proposal of learning to route (\algoLTR~\cite{baranchuk2019learning}) also suggests the opportunity of using machine learning as a new navigation strategy.

\xianzhi{Navigation-based AKNN circumvents the inherent challenge of imperfect range determination encountered in ranging-based AKNN, thereby making it possible to attain both superior retrieval accuracy and higher efficiency. Nevertheless, adjusting navigation information within a proxy graph entails a complex iterative process among neighboring vectors.
}

%Navigation-based AKNN avoids the imperfect range-determination problem of ranging-based AKNN, therefore possible to achieve both higher retrieval accuracy and higher retrieval accuracy. However, modifying the navigation information in a proxy graph involves a complicated workflow of iteration among neighbors.
%
%As we will show in xxx, this leads to xx in the online ingestion case.


%The major difference between different navigation-based AKNN is their various strategies for how to route the navigation path and when to terminate the candidate expansion of neighbors. 
%
 
 
 
%
%Different from using pre-computed ranges, the selected subset \vectorSubset is built from scratch for each query \queryCommand by iteratively appending candidate vectors while navigating from one vector to its neighbors.
\textbf{AKNN Optimizations. }There are various AKNN optimization techniques~\cite{li2023learning,NIPS2008_d58072be,baranchuk2019learning,aguerrebere2024locally,gao2023high}. Despite each of them being specially designed for certain AKNN algorithms or certain distance metrics, we observe that they strategically fall into two categories: i.e., machine-learning-based AKNN~\cite{li2023learning,NIPS2008_d58072be,baranchuk2019learning} and optimized distance computation~\cite{baranchuk2019learning,aguerrebere2024locally}. 
On the one hand, introducing machine learning is promising for both ranging-based~\cite{li2023learning,NIPS2008_d58072be} and navigation-based~\cite{baranchuk2019learning} AKNN. Although there are various designs of 1) neural network structures and 2) loss functions, as summarized in~\cite{li2022deep}, a common key insight is to replace some costly heuristic scan or traverse of vector data with machine learning inference computations, which are typically more straightforward and can also potentially transform the data accessing overhead into mathematical calculations. 
%
On the other hand, optimizing distance computation~\cite{aguerrebere2024locally,gao2023high} is an orthogonal promising strategy besides machine learning. The key insight is to reduce the overhead of calculating and/or comparing distances among vectors, which is a heavy bottleneck for many AKNN algorithms~\cite{gao2023high}. Existing instantiations of this strategy include randomized calculation~\cite{gao2023high} and data compression~\cite{aguerrebere2024locally}.

\textbf{Comparing AKNN on static data.} We refer the reader to the recent detailed surveys and evaluations in ~\cite{li2019approximate,wang2021comprehensive,li2022deep}, which provide comprehensive comparisons of the AKNN algorithms under a wide collection of static data, i.e., including vectors of Image, Text, Audio, and Video. The takeaways from these studies can be summarized as follows. First, AKNN outperforms the brutal-force approach significantly in retrieving efficiency and the reduced accuracy (i.e., measured by recall \recall) is usually acceptable. Second, navigation-based AKNN further outperforms ranging-based AKNN in both retrieving efficiency and accuracy in many datasets.
Third, it is promising to introduce machine learning in optimizing both ranging-based and navigation-based AKNN. 
%
\xianzhi{Different from them, we revisit the effectiveness of AKNN under the more realistic settings of online ingestion. Our conclusions are surprisingly different, and sometimes even contrast to them (Section~\ref{subsec:overall})}


\begin{comment}
\xianzhi{
i.e., to achieve approximate searching on a subset of full data collection and contain correct results in this subset as much as possible. 
AKNN algorithms organize similar vectors together rather than keeping vectors unmanaged as brutal force vector search does. Therefore, the scope is narrowed down into a small subset of the full data collection when accessing vectors, rather than an exhaustive traverse of all. Based on how similar vectors are organized, }
We classify AKNN algorithms into two key categories: Ranging-based and Navigation-based, each further encompassing various sub-variant.

Ranging-based methods establish disjoint ranges across the entire vector space. They conceptually group similar vectors within the same range while segregating distant vectors into separate ranges. The range can be implicitly defined by hash codes or explicitly determined through clustering and space partitioning.
Accessing a range is much more efficient than the full scan, which reduces the searching latency. However, even if using a theoretical optimal range determination, it cannot guarantee that each vector is exclusively located in the same range as its most similar vectors, introducing some level of inaccuracy.
%

In contrast, Navigation-based methods create bidirectional navigation paths that potentially connect all indexed vectors, typically by using a proximity graph. These methods operate on the principle that `a neighbor's neighbor is likely to also be a neighbor'.  Consequently, similar vectors require shorter paths to connect compared to distant vectors. The efficiency lies in searching for similar vectors by iteratively expanding navigation into neighbors' neighbors. Theoretically, optimal navigation can access all desired similar vectors during this iterative expansion without unnecessary navigation into distant ones. However, practical trade-offs, such as searching accuracy, searching latency, and ingestion latency, complicate the implementation.
%
In this paper, ranging-based and navigation-based algorithms are distinguished by the absence or presence of \emph{the bidirectional navigation paths potentially connecting all indexed vectors}, respectively. The existence of these paths is vital for achieving higher theoretical accuracy, and their significant impact on practical performance will be further evaluated in Section xxx.





\subsection{-- Some Preliminary Studies to motivate this work --}
1) Re-build from scratch? 
2) ...
\end{comment}

==> BenchmarkSystems/Architecture.tex <==
\subsection{System Architecture}
\label{subsec:system_architecture}
Outline the overall architecture of \system, detailing the ingestion frontend, evaluation backend, and their interdependencies.

\input{BenchmarkSystems/Frontend}

\input{BenchmarkSystems/Backend}





==> BenchmarkSystems/Backend.tex <==
\subsubsection{Evaluation Backend}
\label{subsubsec:evaluation_backend}
Describe the backend evaluation setup, including the AKNN approaches evaluated and the criteria for their testing.

This section details the evaluation backend of \system. We first discuss the evaluated AKNN approaches, then their adaptations to dynamic ingestion, and finally the optional optimization techniques. 
\subsubsection{Evaluated AKNN Approaches}
\label{subsub:algos}
We discussed the evaluated AKNN approaches in this part. We first illustrate the common concepts of AKNN, and next divide them into two categories based on their different approximation strategies. Please refer to~\ref{} for more discussions of each strategy.

\textbf{AKNN concepts.}
Nearest Neighbor Search (NNS) is a fundamental operation in the data science community~\cite{manning2008introduction, han2011data, ricci2011introduction, indyk1998approximate, weber1998quantitative, arya1998optimal, gionis1999similarity}. Specifically, given a query \queryCommand, NNS aims at searching \annk \emph{closest} vectors among all of the ingested vectors, denoted as \vectorSet. There are various \emph{distance measures} to define the ``closest'', and two common measures are L2 distance~\cite{li2019approximate} and inner product distance~\cite{aguerrebere2024locally}. \system supports both, and inner product is the default for AI applications.

Intuitively, searching for the closet requires exhaustive traversal over \vectorSet to compute distance and compare the vectors, and such an exact but brutal force approach is included in \system as the baseline (denoted as \algoBF for short in the following).
%
AKNN aims to avoid exhaustive traversal over \vectorSet by introducing approximations. Specifically, it selects a subset from \vectorSet, denoted as \vectorSubset (i.e., $\vectorSubsetInEq \subseteq \vectorSetInEq$). 
By \vectorSubset-based searching instead of a full scan of \vectorSet, AKNN is considered to achieve superior retrieval efficiency than \algoBF.
%
%The result of AKNN is represented by \resulSetAKNN, which contains \annk vectors from the subset \vectorSubset.
%
%The set \resulSetAKNN typically differs from the exact search result \resulSet, and the disparity between \resulSetAKNN and \resulSet serves as the accuracy metric for AKNN, often referred to as ``recall'' and denoted as \recall. Specifically, \recall is a fractional value calculated as $\recallInEq = \frac{|\resulSetAKNNInEq \cap \resulSetInEq|}{\annkInEq}$.

\begin{table}[]
\centering
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{|c|l|l|}
\hline
\multicolumn{1}{|c|}{\textit{Category}} & \textit{Algorithm Name}                & \textit{Descriptions}                                                                                             \\ \hline
\multirow{6}{*}{Ranging-based}        
& \algoLSH~\cite{gionis1999similarity}   & Data-independednt hashing to determine ranges                                                                     \\ \cline{2-3} 
 & \algoFlann~\cite{muja2014scalable}     & Space partition to determine ranges                                                                               \\ \cline{2-3} 
                                        & \algoPQ~\cite{jegou2010product}        & Product quantization to determin ranges                                                                           \\ \cline{2-3} 
                                        & \algoIVFPQ~\cite{jegou2010product}     & Hierachical optimization over \algoPQ                                                                             \\ \cline{2-3} 
                                       
                                        & \algoOnlinePQ~\cite{xu2018online}        & Incrementally update centroids of \algoPQ 
                                                                                  \\ \hline
\multirow{5}{*}{Navigation-based}       & \algoNSW~\cite{malkov2014approximate}  & Delaunay Graph for navigation                                                                                     \\ \cline{2-3} 
                                        & \algoNNDecent~\cite{dong2011efficient} & K-Nearest Neighbor Graph for navigation                                                                           \\ \cline{2-3} 
                                        & \algoDPG~\cite{li2019approximate}      & \begin{tabular}[c]{@{}l@{}}K-Nearest Neighbor Graph and Relative Neighborhood Graph\\ for Navigation\end{tabular} \\ \cline{2-3} 
                                        & \algoNSG~\cite{fu2019fast}      & \begin{tabular}[c]{@{}l@{}} Optimized vertex assignment compared with \algoDPG \end{tabular} \\ \cline{2-3} 
                                        & \algoHNSW~\cite{malkov2018efficient}   & Hiearchical construction of \algoNSW                                                                                                                                                       \\ \hline
\end{tabular}
}
\caption{Studied AKNN algorithms}
\label{tab:algosList}
\end{table}

Depending on the major difference of how \vectorSubset is generated, 
we broadly classify the state-of-the-art ANNS algorithms into two
main categories in the following: \emph{ranging-based} and \emph{navigation-based}. We summarized the representative examples of each category in Table~\ref{tab:algosList}. 
%We discuss the existing comparison results of these categories at the end of this section.


%This paper proposes the first comprehensive benchmark study to revisit vector indexing under dynamic ingestion. It evaluates numerous vector indexing algorithms, with a focus on those allowing or specifically designed for dynamic updates. Our study encompasses various datasets and updating patterns. 
\textbf{Ranging-based AKNN.} Ranging-based AKNN utilizes pre-computed range division of \vectorSet regardless of the specific \queryCommand.
Specifically, it firstly divides \vectorSet into disjoint ranges $D_1, D_2,...,D_n$. When encountering a \queryCommand, the \vectorSubset is directly picked by using a pre-computed range (e.g., $\vectorSubsetInEq = D_1$), or using the union of several ranges (e.g., $\vectorSubsetInEq = D_1 \cup D_2$). \system covers a wide range of range-based AKNN, from the earliest \algoLSH to the one specially designed for dynamic data ingestion case, i.e., \algoOnlinePQ. 


\textbf{Navigation-based AKNN.} 
The navigation-based AKNN method establishes a navigational connection to associate each ingested vector in the data collection \vectorSet with its similar vectors, often achieved by using a proximity graph.
%
In contrast to employing pre-computed ranges, the chosen subset (\vectorSubset) is constructed anew for every query (\queryCommand) by iteratively adding candidate vectors during the navigation process from one vector to its neighboring vectors. 
The primary distinction among various navigation-based AKNN approaches lies in their diverse strategies for determining the navigation path and deciding when to terminate the expansion of candidate neighbors.
We include various popular institutions in the proximity graph, such as K-Nearest Neighbor Graph (\algoNNDecent) and hierarchical approximate Delaunay Graph (\algoHNSW).
%

\subsubsection{Adapating AKNN to Dynamic Ingestion}
Most AKNNs are mainly intended for static data, and we summarize how they are adapted to dynamic ingestion in this part.

\textbf{To Adapt AKNN with Minor Changes.} We observe that some of the AKNN inherently build their index in an incremental and one-pass manner, without any repeated scan or reference on the yet-to-come data, specifically, \algoLSH, \algoNSW and \algoHNSW. Moreover, \algoOnlinePQ is intentionally designed for ingesting dynamic data. These algorithms require no significant changes to be adapted in the dynamic ingestion case, and we just align their API and I/O data structure in our codebase.

\textbf{To Adapt AKNN with Enforced Assumptions.} 
\algoPQ and \algoIVFPQ also ingest data in an incremental and one-pass manner. Nevertheless, this process additionally relies on an established knowledge of data distributions. 
The knowledge-building process requires multiple scans on full data collection and involves notoriously large overhead, e.g., xxx for \algoIVFPQ over xxx data scale. Therefore, 
we set up the knowledge for them only at the offline stage and assume it is still valid in dynamic ingestion. Note that, any overhead in the offline stage is excluded from our evaluation.

\textbf{To Adapt AKNN with Algorithm Modifications.} 
The rest of the evaluated AKNN, i.e., \algoNNDecent,  \algoDPG and \algoNSG are highly specialized for static data, specifically, xxxxx. To adapt them into dynamic ingestion case, we xxxx.
\xianzhi{
---
write your own analysis and optimizations here
@zhuoyan @xinjing 
} 
\algoNSG (Navigable Spreading-out Graph) depends on a pre-built graph by brute force. A navigation point would be selected randomly as the entry point for subsequent insertion and search. For the rest of the points, all neighbor candidates would be searched and linked starting from the navigation point so that all sub-graphs are connected with the navigation point. To adapt \algoNSG into dynamic ingestion case, the ingested points would go through a similar process as those from the pre-built graph, that they carry out a global neighbor search from the navigation point and update the graph structure accordingly.


\subsubsection{AKNN Optimizations}
\label{subsub:aknn_opts}
There are various AKNN optimization techniques~\cite{li2023learning,NIPS2008_d58072be,baranchuk2019learning,aguerrebere2024locally,gao2023high}. Despite each of them being specially designed for certain AKNN algorithms or certain distance metrics, we observe that they strategically fall into two categories: i.e., machine-learning-based AKNN~\cite{li2023learning,NIPS2008_d58072be,baranchuk2019learning} and optimized distance computation~\cite{baranchuk2019learning,aguerrebere2024locally}. 

\textbf{Machine-learning-based AKNN.}
Introducing machine learning is promising for both ranging-based~\cite{li2023learning,NIPS2008_d58072be} and navigation-based~\cite{baranchuk2019learning} AKNN. Although there are various designs of 1) neural network structures and 2) loss functions, as summarized in~\cite{li2022deep}, a common key insight is to replace some costly heuristic scan or traverse of vector data with machine learning inference computations, which are typically more straightforward and can also potentially transform the data accessing overhead into mathematical calculations. 
\xianzhi{Thanks to the alignment of LibTorch/Pytorch ecosystem (Section~\ref{subsub:apis}). 
\system supports arbitrary standardised neural network classes derived from \emph{torch::nn::Module}, arbitrary 
derivable tensor loss functions, and common optimizers of LibTorch such as \emph{torch::optim::Adam}, which paves the way for future adventures of optimizing AKNN through machine learning.}



%
\textbf{Optimized Distance Computation}
On the other hand, optimizing distance computation~\cite{aguerrebere2024locally,gao2023high} is an orthogonal promising strategy besides machine learning. The key insight is to reduce the overhead of calculating and/or comparing distances among vectors, which is a heavy bottleneck for many AKNN algorithms~\cite{gao2023high}. Existing instantiations of this strategy include randomized calculation~\cite{gao2023high} and data compression~\cite{aguerrebere2024locally}. Both of them are integrated in the backend of \system.
\xianzhi{--@xinjing @zhuoyan write more if we have.}



==> BenchmarkSystems/Challenges.tex <==
\section{Dynamic Data Ingestion Challenges}
\label{subsec_challenges}
Despite the rich literature and comprehensive evaluation of AKNN under static data scenarios, ``how AKNN performs under dynamic data ingestion challenges'' is still an open question. We illustrate the problem significance through a motivation example, and then highlight the detailed challenges raised by ingestion efficiency and distribution shifts.

\begin{figure}[t]
\begin{minipage}[a]{\textwidth} 
\centering
            \begin{minipage}[b]{0.4\textwidth}
        \includegraphics*[width=0.99\textwidth]{figures/e1.pdf}
        \caption{ AKNN in RAG system.}
    \label{fig:intro_1}
    \end{minipage}    
        \begin{minipage}[b]{0.59\textwidth}
        \includegraphics*[width=0.99\textwidth]{figures/e2.pdf}
        \caption{AKNN under dynamic ingestion challenges.}
    \label{fig:intro_2}
    \end{minipage}    
     
\end{minipage}
\end{figure}

\textbf{Motivation Example.}
Consider an advanced RAG system implemented in the data center of a giant brand for its real-time decision-making and customer service ~\cite{pandya2023automating,khan2023impact} (Figure~\ref{fig:intro_1}).
%
This system continuously receives new content from customers at a rate of $4K\sim6K$ per second ~\cite{sundaram2013streaming,tweetsSpeed}, consisting of suggestions, queries, and complaints. Many posts, particularly complaints, are vague and emotionally charged, making it challenging for the system to accurately extract user feedback using simple methods like regular expressions on a relational database. 
%
For instance, an angry user complained that disinfectant product A is apple juice for germs, indicating A is poor in the kitchen. 
%
Moreover, due to constantly evolving product lines (e.g., disinfectant A and sleeping pills B), user sentiments, and specific needs or criticisms, relying solely on a pre-trained large language model (LLM) is insufficient. Consequently, the RAG system utilizes both the database of ingested user posts and the extensive linguistic capabilities of an LLM to discern prevalent customer sentiments and generate suggestions based on real-time public opinion synthesis.
%
This task is a common summarization in RAG literature, as described in~\cite{lyu2024crud}. 

In this system, AKNN is pivotal for quickly indexing vectorized posts, enabling the generation of dependable summarizations and guiding subsequent actions or responses~\cite{gao2023retrieval, aguerrebere2024locally, lewis2020retrieval}. For example, AKNN is used to retrieve recent feedback about disinfectant A (coloured grey in Figure~\ref{fig:intro_1}), allowing the LLM to analyze and summarize the common satisfactions and criticisms noted by users.

\textbf{The Ingestion Efficiency Challenge.}
The AKNN is expected to ingest all of the necessary data collection, such that ending applications like aforementioned RAG have correct data collection to generate useful results. However, this rapid influx of data poses significant constraints on the time and computational resources available for processing. These constraints, often overlooked in AKNN literature, critically limit the system's ability to maintain an up-to-date index and effectively serve user posts. When the processing capability of AKNN algorithms falls behind the data flow, an unmanageable backlog can form, potentially growing indefinitely~\cite{cidon2015tiered,andrews2004scheduling,fowler1991local,arun2018copa}. Temporarily halting data input until the backlog is cleared is not feasible, given the limited storage for pending data. Consequently, AKNN is forced to discard incoming information,
degrading search quality and leading to unuseful system output, i.e., Figure~\ref{fig:intro_2}-a).

\textbf{The Distribution Shift Challenge.}
The efficiency of AKNN is further compromised by shifts in data distribution \cite{aguerrebere2024locally}. As shown in Figure \ref{fig:intro_2}-b), the ``germ's juice'' complaints about disinfectant A, characterized by anger and expressed implicitly (i.e., coloured in red), fall outside the distribution range of typical data collection (i.e., coloured in white), which is generally not such emotion-charged.
%
Furthermore, there is no prior knowledge about the \emph{occurrence position} or \emph{occurrence intensity} of these shifts, as data continuously arrive from external sources.
%
Under these conditions, AKNN must still manage to provide sufficiently accurate searches to ensure the system remains comprehensive, rather than indexing wrongly and generating biased results like Figure \ref{fig:intro_2}-b).

==> BenchmarkSystems/DataInput.tex <==
\subsection{Data Input}
We discuss the data input part of \system in this section, including the datasets and input admission control mechanisms.
\begin{table}[t]
\centering
    \centering
    \resizebox{0.7\textwidth}{!}{%
   \begin{tabular}{|l|l|l|l|}
\hline
\multirow{7}{*}{Real-world} & \textbf{Name}                                                   & \textbf{Description} & \textbf{Dimension} \\ \cline{2-4} 
                            & \Glove~\cite{li2019approximate}                                 & Text embedding       & $100$              \\ \cline{2-4} 
                            & \SIFT~\cite{li2019approximate}                                  & Image                & $128$              \\ \cline{2-4} 
                            & \Msong~\cite{li2019approximate}                                 & Audio                & $4208$             \\ \cline{2-4} 
                            & \Sun~\cite{li2019approximate}                                   & Image                & $512$              \\ \cline{2-4} 
                            & \DPR~\cite{aguerrebere2024locally}                              & Text embedding       & $768$              \\ \cline{2-4} 
                            & \Trevi~\cite{li2019approximate}                                 & Image                & $4096$             \\ \hline
\multirow{2}{*}{Synthetic}  & \Random~\cite{Pytorch}                                          & i.i.d values         & Adjustable         \\ \cline{2-4} 
                            & \Wte~\cite{aguerrebere2024locally,warthunderWiki,loper2002nltk} & Text embedding       & $768$              \\ \hline
\end{tabular}
}
\caption{Datasets.}
\label{tab:realworld_workloads}
\end{table}

\subsubsection{Datasets} 
\label{subsub:datasets}
We follow state-of-art to cover a wide range of real-world and synthetic datasets, besides, we propose a new synthetic dataset, namely \Wte (\textbf{W}ar\textbf{T}hunder \textbf{E}mbeddings), to investigate the impacts of distribution shifts.

\textbf{Datasets from Existing Works.}
Following the methodologies outlined in ~\cite{li2019approximate,aguerrebere2024locally}, we encompass a wide variety of \emph{real-world workloads} as detailed in Table~\ref{tab:realworld_workloads}, which span across several application domains, including text embeddings (\DPR) and image processing (\Trevi). The \DPR dataset was reconstructed using the source code and corpus provided by ~\cite{aguerrebere2024locally}, whereas the remaining datasets were obtained from ~\cite{li2019approximate}. As a preliminary step, we normalize each dataset using the \emph{torch::norm} function from LibTorch~\cite{Pytorch} to ensure that the values range between -1 and 1.

In addition to these real-world datasets, we include a 
straightforward synthetic dataset \Random from LibTorch~\cite{Pytorch}. The \Random dataset consists of values generated by the \emph{torch::random} function, which produces a sequence of independent and identically distributed (i.i.d.) uniform values between $0$ and $1$. This approach allows for the configuration of dimensions and volumes of vectors to suit various needs, such as investigating ``the curse of dimensions''.

\textbf{A New Synthetic Dataset \Wte for Distribution Shifts.}
\Wte utilize the \DPR-like embeddings of synthetic sentences to  
tune both the occurrence position and general intensity of distribution shifts (Section~\ref{subsec_challenges}) in \Wte. 
The nouns in sentences have distinct categories as detailed in a video game ~\cite{warthunderWiki}.
To manipulate the occurrence position, we generate vector embeddings from one category of nouns and subsequently transition to vector embeddings of another noun category, and the starting position of a new category. To explore variations in the general intensity of distribution shifts, 
we construct the entire sentence collection using nouns related to one category. Subsequently, we induce a distribution shift starting at a fixed position and randomly replacing the subject noun with a specific noun, which belongs to a different category. The resulting sentence, contaminated by this shift, is then used to generate embeddings. 
This process emulates real-world scenarios where a sudden emergence of a prominent topic occurs, and the intensity of the shift is adjusted by varying the probability of word contamination. Please refer to~\ref{} for more details.

\subsubsection{Input Admission Control Mechanisms} 
\label{subsub:input_ctl}
The real-world challenge of ingestion efficiency means that we cannot ensure that all data are fully ingested by AKNN before processing, e.g., Figure~\ref{fig:intro_2}-a). To reflect this scenario, we introduced a specific source in \system. This source operates independently of both frontend interfaces and backend components and it is solely driven by a configurable high-resolution clock that releases loaded data at a constant rate, typically set at $4K$ rows per second by default. If AKNN processes data more slowly than this rate, excess data is naturally dropped to avoid congestion.

In contrast to the default drop-on-congestion approach, we have also implemented a version where congested data is temporarily stored in an in-memory queue, allowing AKNN to eventually process all incoming data. 
Note that, this contradicting version is an oversimplification of real-world applications as data sources often cannot be paused by the AKNN side, and such queuing could quickly exhaust available memory. Moreover, as detailed in our technical report ~\ref{}, this method of queuing actually further decreases ingestion efficiency, even under the held assumption of its practicality.

==> BenchmarkSystems/Frontend.tex <==
\subsubsection{Ingestion Frontend}
\label{subsubsec:ingestion_frontend}
Discuss the design and functionality of the ingestion frontend, including data agglomeration and API specifics.



The section details the ingestion frontend design of \system, including the agglomeration and API.
\subsubsection{Agglomeration}
\label{subsub:batch}
\system employs a micro-batching technique to agglomerate data, which operates independently of the backend algorithms or their optimizations. The data science community has widely recognized the advantages of micro-batching for managing and processing large datasets effectively, although the motivation and purposes can be different. Micro-batching allows for segmenting extensive datasets into smaller, manageable units, which supports more frequent updates to machine learning model parameters, thereby promoting faster convergence~\cite{huang2019gpipe,yuan2022decentralized}. On the other hand, opting for a strategy that aggregates data in larger batches, rather than processing streams eagerly, can significantly improve the throughput of online database systems~\cite{zhang2021parallelizing}. Inspired by these research findings, we have made the micro-batch size configurable within our system to enable more detailed evaluations, as discussed in Section~\ref{}.
%experimented with adjusting the micro-batch size for AKNN data ingestion from 200 to 50,000 and observed the effects on query latency. The resulting query recall and latency are demonstrated in Figure~\ref{fig:batch}.

\subsubsection{API and Alignments}
\label{subsub:apis}
We aligned all of the accessing API in a unified way, including 1) initialization processes, 2)loading offline data, 3) online ingestion, and 4) vector search. These APIs are fully compatible with LibTorch and PyTorch~\cite{Pytorch}, which are widely used in the data science community, and they are available in both C++ and Python. Behind the API are our further alignments during the implementation. Particularly, 1) the unified C++ codebase, 2) static compilation, and 3) interfaces based on \emph{torch::Tensor}. Please refer to our codebase documents~\ref{} for their details.


==> EvaluationShort/LargeTables.tex <==
% \subsection{Supplementary Tables}
% We present the supplementary data tables in this section, please rotate the next pages clockwise by 90 degrees before examining them.
% \label{subsec:large_tables}
\begin{sidewaystable}[]
\centering
\begin{minipage}{\textwidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|ll|llllll|llllll|llllll|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{Algorithms}}                                & \multicolumn{6}{l|}{Propotion of Pending Write Latency (\%)}                                                                                                                                                 & \multicolumn{6}{l|}{Pending Write Latency ($\times 1000 ms$)}                                                                                                                                                       & \multicolumn{6}{l|}{Vector Search Latency ($\times 1000 ms$)}                                                                                                                                              \\ \cline{3-20} 
\multicolumn{2}{|l|}{}                                  & \multicolumn{1}{l|}{\Glove}         & \multicolumn{1}{l|}{\SIFT}          & \multicolumn{1}{l|}{\Msong}         & \multicolumn{1}{l|}{\Sun}           & \multicolumn{1}{l|}{\DPR}           & \Trevi         & \multicolumn{1}{l|}{\Glove}          & \multicolumn{1}{l|}{\SIFT}          & \multicolumn{1}{l|}{\Msong}          & \multicolumn{1}{l|}{\Sun}            & \multicolumn{1}{l|}{\DPR}            & \Trevi            & \multicolumn{1}{l|}{\Glove}        & \multicolumn{1}{l|}{\SIFT}         & \multicolumn{1}{l|}{\Msong}        & \multicolumn{1}{l|}{\Sun}          & \multicolumn{1}{l|}{\DPR}           & \Trevi           \\ \hline
\multicolumn{2}{|l|}{\textbf{\algoBF}}                                           & \multicolumn{1}{l|}{\textbf{83.29}} & \multicolumn{1}{l|}{\textbf{79.50}} & \multicolumn{1}{l|}{\textbf{73.13}} & \multicolumn{1}{l|}{\textbf{78.20}} & \multicolumn{1}{l|}{\textbf{63.32}} & \textbf{59.96} & \multicolumn{1}{l|}{\textbf{0.36}}   & \multicolumn{1}{l|}{\textbf{0.35}}  & \multicolumn{1}{l|}{\textbf{0.44}}   & \multicolumn{1}{l|}{\textbf{0.54}}   & \multicolumn{1}{l|}{\textbf{0.48}}   & \textbf{1.51}     & \multicolumn{1}{l|}{\textbf{0.07}} & \multicolumn{1}{l|}{\textbf{0.09}} & \multicolumn{1}{l|}{\textbf{0.16}} & \multicolumn{1}{l|}{\textbf{0.15}} & \multicolumn{1}{l|}{\textbf{0.28}}  & \textbf{1.01}    \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{Ranging-based}}    & \algoLSH               & \multicolumn{1}{l|}{91.08}          & \multicolumn{1}{l|}{86.38}          & \multicolumn{1}{l|}{74.99}          & \multicolumn{1}{l|}{30.49}          & \multicolumn{1}{l|}{89.10}          & 1.11           & \multicolumn{1}{l|}{0.16}            & \multicolumn{1}{l|}{0.19}           & \multicolumn{1}{l|}{0.17}            & \multicolumn{1}{l|}{0.13}            & \multicolumn{1}{l|}{0.17}            & 0.13              & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.03}          & \multicolumn{1}{l|}{0.06}          & \multicolumn{1}{l|}{0.29}          & \multicolumn{1}{l|}{0.02}           & 11.83            \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoFlann             & \multicolumn{1}{l|}{98.61}          & \multicolumn{1}{l|}{98.70}          & \multicolumn{1}{l|}{98.99}          & \multicolumn{1}{l|}{98.90}          & \multicolumn{1}{l|}{98.14}          & 97.48          & \multicolumn{1}{l|}{1.07}            & \multicolumn{1}{l|}{1.16}           & \multicolumn{1}{l|}{1.83}            & \multicolumn{1}{l|}{1.63}            & \multicolumn{1}{l|}{1.24}            & 2.62              & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.02}           & 0.07             \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoPQ                & \multicolumn{1}{l|}{99.67}          & \multicolumn{1}{l|}{99.62}          & \multicolumn{1}{l|}{99.55}          & \multicolumn{1}{l|}{99.61}          & \multicolumn{1}{l|}{99.61}          & 99.53          & \multicolumn{1}{l|}{353.26}          & \multicolumn{1}{l|}{350.25}         & \multicolumn{1}{l|}{356.80}          & \multicolumn{1}{l|}{362.51}          & \multicolumn{1}{l|}{360.10}          & 412.80            & \multicolumn{1}{l|}{1.17}          & \multicolumn{1}{l|}{1.33}          & \multicolumn{1}{l|}{1.60}          & \multicolumn{1}{l|}{1.41}          & \multicolumn{1}{l|}{1.40}           & 1.97             \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoIVFPQ             & \multicolumn{1}{l|}{99.67}          & \multicolumn{1}{l|}{97.20}          & \multicolumn{1}{l|}{99.52}          & \multicolumn{1}{l|}{86.56}          & \multicolumn{1}{l|}{99.55}          & 99.16          & \multicolumn{1}{l|}{392.11}          & \multicolumn{1}{l|}{2.05}           & \multicolumn{1}{l|}{398.64}          & \multicolumn{1}{l|}{2.47}            & \multicolumn{1}{l|}{407.78}          & 500.24            & \multicolumn{1}{l|}{1.29}          & \multicolumn{1}{l|}{0.06}          & \multicolumn{1}{l|}{1.92}          & \multicolumn{1}{l|}{0.38}          & \multicolumn{1}{l|}{1.83}           & 4.22             \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \textbf{\algoOnlinePQ} & \multicolumn{1}{l|}{\textbf{84.43}} & \multicolumn{1}{l|}{\textbf{79.47}} & \multicolumn{1}{l|}{\textbf{94.38}} & \multicolumn{1}{l|}{\textbf{99.39}} & \multicolumn{1}{l|}{\textbf{99.14}} & \textbf{99.15} & \multicolumn{1}{l|}{\textbf{1.35}}   & \multicolumn{1}{l|}{\textbf{0.96}}  & \multicolumn{1}{l|}{\textbf{3.17}}   & \multicolumn{1}{l|}{\textbf{382.15}} & \multicolumn{1}{l|}{\textbf{392.14}} & \textbf{19.03}    & \multicolumn{1}{l|}{\textbf{0.25}} & \multicolumn{1}{l|}{\textbf{0.25}} & \multicolumn{1}{l|}{\textbf{0.19}} & \multicolumn{1}{l|}{\textbf{2.33}} & \multicolumn{1}{l|}{\textbf{3.41}}  & \textbf{0.16}    \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{Navigation-based}} & \textbf{\algoHNSW}     & \multicolumn{1}{l|}{\textbf{99.97}} & \multicolumn{1}{l|}{\textbf{99.80}} & \multicolumn{1}{l|}{\textbf{99.96}} & \multicolumn{1}{l|}{\textbf{99.98}} & \multicolumn{1}{l|}{\textbf{88.94}} & \textbf{86.87} & \multicolumn{1}{l|}{\textbf{117.72}} & \multicolumn{1}{l|}{\textbf{15.83}} & \multicolumn{1}{l|}{\textbf{151.52}} & \multicolumn{1}{l|}{\textbf{584.60}} & \multicolumn{1}{l|}{\textbf{615.08}} & \textbf{11698.58} & \multicolumn{1}{l|}{\textbf{0.04}} & \multicolumn{1}{l|}{\textbf{0.03}} & \multicolumn{1}{l|}{\textbf{0.06}} & \multicolumn{1}{l|}{\textbf{0.11}} & \multicolumn{1}{l|}{\textbf{76.49}} & \textbf{1767.90} \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoNSW               & \multicolumn{1}{l|}{91.40}          & \multicolumn{1}{l|}{91.30}          & \multicolumn{1}{l|}{99.98}          & \multicolumn{1}{l|}{89.53}          & \multicolumn{1}{l|}{90.48}          & 88.04          & \multicolumn{1}{l|}{1721.73}         & \multicolumn{1}{l|}{212.89}         & \multicolumn{1}{l|}{454.59}          & \multicolumn{1}{l|}{689.47}          & \multicolumn{1}{l|}{1077.06}         & 6205.80           & \multicolumn{1}{l|}{161.95}        & \multicolumn{1}{l|}{20.28}         & \multicolumn{1}{l|}{0.09}          & \multicolumn{1}{l|}{80.61}         & \multicolumn{1}{l|}{113.37}         & 843.11           \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoNSG               & \multicolumn{1}{l|}{99.97}          & \multicolumn{1}{l|}{93.73}          & \multicolumn{1}{l|}{94.33}          & \multicolumn{1}{l|}{99.97}          & \multicolumn{1}{l|}{99.94}          & 94.80          & \multicolumn{1}{l|}{30.62}           & \multicolumn{1}{l|}{302.93}         & \multicolumn{1}{l|}{378.95}          & \multicolumn{1}{l|}{46.18}           & \multicolumn{1}{l|}{48.48}           & 1196.68           & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{20.26}         & \multicolumn{1}{l|}{22.80}         & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.03}           & 65.63            \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoNNDecent          & \multicolumn{1}{l|}{98.15}          & \multicolumn{1}{l|}{99.07}          & \multicolumn{1}{l|}{98.77}          & \multicolumn{1}{l|}{98.27}          & \multicolumn{1}{l|}{98.83}          & 97.46          & \multicolumn{1}{l|}{30.01}           & \multicolumn{1}{l|}{15.24}          & \multicolumn{1}{l|}{5.27}            & \multicolumn{1}{l|}{6.49}            & \multicolumn{1}{l|}{39.90}           & 19.71             & \multicolumn{1}{l|}{0.57}          & \multicolumn{1}{l|}{0.14}          & \multicolumn{1}{l|}{0.07}          & \multicolumn{1}{l|}{0.11}          & \multicolumn{1}{l|}{0.47}           & 0.51             \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoDPG               & \multicolumn{1}{l|}{98.68}          & \multicolumn{1}{l|}{98.69}          & \multicolumn{1}{l|}{98.26}          & \multicolumn{1}{l|}{98.11}          & \multicolumn{1}{l|}{99.33}          & 98.29          & \multicolumn{1}{l|}{18.56}           & \multicolumn{1}{l|}{19.53}          & \multicolumn{1}{l|}{603.45}          & \multicolumn{1}{l|}{679.32}          & \multicolumn{1}{l|}{86.93}           & 5452.70           & \multicolumn{1}{l|}{0.25}          & \multicolumn{1}{l|}{0.26}          & \multicolumn{1}{l|}{10.67}         & \multicolumn{1}{l|}{13.11}         & \multicolumn{1}{l|}{0.59}           & 94.85            \\ \hline
\end{tabular}
}
\caption{Overall Comparison. Full table of both Inner Product and L2 Distance.}
\label{tab:e2e_ip_full}
\end{minipage}
\begin{minipage}{\textwidth}
\centering
 \resizebox{\textwidth}{!}{%
\begin{tabular}{|ll|llllll|llllll|llllll|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{Algorithms}}                                & \multicolumn{6}{l|}{Propotion of Pending Write Latency (\%)}                                                                                                                                                 & \multicolumn{6}{l|}{Pending Write Latency ($\times 1000 ms$)}                                                                                                                                                       & \multicolumn{6}{l|}{Vector Search Latency ($\times 1000 ms$)}                                                                                                                                              \\ \cline{3-20} 
\multicolumn{2}{|l|}{}                                  & \multicolumn{1}{l|}{\Glove}         & \multicolumn{1}{l|}{\SIFT}          & \multicolumn{1}{l|}{\Msong}         & \multicolumn{1}{l|}{\Sun}           & \multicolumn{1}{l|}{\DPR}           & \Trevi         & \multicolumn{1}{l|}{\Glove}          & \multicolumn{1}{l|}{\SIFT}          & \multicolumn{1}{l|}{\Msong}          & \multicolumn{1}{l|}{\Sun}            & \multicolumn{1}{l|}{\DPR}            & \Trevi            & \multicolumn{1}{l|}{\Glove}        & \multicolumn{1}{l|}{\SIFT}         & \multicolumn{1}{l|}{\Msong}        & \multicolumn{1}{l|}{\Sun}          & \multicolumn{1}{l|}{\DPR}           & \Trevi           \\ \hline
\multicolumn{2}{|l|}{\textbf{\algoBF}}                                           & \multicolumn{1}{l|}{\textbf{83.29}} & \multicolumn{1}{l|}{\textbf{79.50}} & \multicolumn{1}{l|}{\textbf{73.13}} & \multicolumn{1}{l|}{\textbf{78.20}} & \multicolumn{1}{l|}{\textbf{63.32}} & \textbf{59.96} & \multicolumn{1}{l|}{\textbf{0.36}}   & \multicolumn{1}{l|}{\textbf{0.35}}  & \multicolumn{1}{l|}{\textbf{0.44}}   & \multicolumn{1}{l|}{\textbf{0.54}}   & \multicolumn{1}{l|}{\textbf{0.48}}   & \textbf{1.51}     & \multicolumn{1}{l|}{\textbf{0.07}} & \multicolumn{1}{l|}{\textbf{0.09}} & \multicolumn{1}{l|}{\textbf{0.16}} & \multicolumn{1}{l|}{\textbf{0.15}} & \multicolumn{1}{l|}{\textbf{0.28}}  & \textbf{1.01}    \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{Ranging-based}}    & \algoLSH               & \multicolumn{1}{l|}{91.08}          & \multicolumn{1}{l|}{86.38}          & \multicolumn{1}{l|}{74.99}          & \multicolumn{1}{l|}{30.49}          & \multicolumn{1}{l|}{89.10}          & 1.11           & \multicolumn{1}{l|}{0.16}            & \multicolumn{1}{l|}{0.19}           & \multicolumn{1}{l|}{0.17}            & \multicolumn{1}{l|}{0.13}            & \multicolumn{1}{l|}{0.17}            & 0.13              & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.03}          & \multicolumn{1}{l|}{0.06}          & \multicolumn{1}{l|}{0.29}          & \multicolumn{1}{l|}{0.02}           & 11.83            \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoFlann             & \multicolumn{1}{l|}{98.61}          & \multicolumn{1}{l|}{98.70}          & \multicolumn{1}{l|}{98.99}          & \multicolumn{1}{l|}{98.90}          & \multicolumn{1}{l|}{98.14}          & 97.48          & \multicolumn{1}{l|}{1.07}            & \multicolumn{1}{l|}{1.16}           & \multicolumn{1}{l|}{1.83}            & \multicolumn{1}{l|}{1.63}            & \multicolumn{1}{l|}{1.24}            & 2.62              & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.02}           & 0.07             \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoPQ                & \multicolumn{1}{l|}{99.67}          & \multicolumn{1}{l|}{99.62}          & \multicolumn{1}{l|}{99.55}          & \multicolumn{1}{l|}{99.61}          & \multicolumn{1}{l|}{99.61}          & 99.53          & \multicolumn{1}{l|}{353.26}          & \multicolumn{1}{l|}{350.25}         & \multicolumn{1}{l|}{356.80}          & \multicolumn{1}{l|}{362.51}          & \multicolumn{1}{l|}{360.10}          & 412.80            & \multicolumn{1}{l|}{1.17}          & \multicolumn{1}{l|}{1.33}          & \multicolumn{1}{l|}{1.60}          & \multicolumn{1}{l|}{1.41}          & \multicolumn{1}{l|}{1.40}           & 1.97             \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoIVFPQ             & \multicolumn{1}{l|}{99.67}          & \multicolumn{1}{l|}{97.20}          & \multicolumn{1}{l|}{99.52}          & \multicolumn{1}{l|}{86.56}          & \multicolumn{1}{l|}{99.55}          & 99.16          & \multicolumn{1}{l|}{392.11}          & \multicolumn{1}{l|}{2.05}           & \multicolumn{1}{l|}{398.64}          & \multicolumn{1}{l|}{2.47}            & \multicolumn{1}{l|}{407.78}          & 500.24            & \multicolumn{1}{l|}{1.29}          & \multicolumn{1}{l|}{0.06}          & \multicolumn{1}{l|}{1.92}          & \multicolumn{1}{l|}{0.38}          & \multicolumn{1}{l|}{1.83}           & 4.22             \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \textbf{\algoOnlinePQ} & \multicolumn{1}{l|}{\textbf{84.43}} & \multicolumn{1}{l|}{\textbf{79.47}} & \multicolumn{1}{l|}{\textbf{94.38}} & \multicolumn{1}{l|}{\textbf{99.39}} & \multicolumn{1}{l|}{\textbf{99.14}} & \textbf{99.15} & \multicolumn{1}{l|}{\textbf{1.35}}   & \multicolumn{1}{l|}{\textbf{0.96}}  & \multicolumn{1}{l|}{\textbf{3.17}}   & \multicolumn{1}{l|}{\textbf{382.15}} & \multicolumn{1}{l|}{\textbf{392.14}} & \textbf{19.03}    & \multicolumn{1}{l|}{\textbf{0.25}} & \multicolumn{1}{l|}{\textbf{0.25}} & \multicolumn{1}{l|}{\textbf{0.19}} & \multicolumn{1}{l|}{\textbf{2.33}} & \multicolumn{1}{l|}{\textbf{3.41}}  & \textbf{0.16}    \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{Navigation-based}} & \textbf{\algoHNSW}     & \multicolumn{1}{l|}{\textbf{99.97}} & \multicolumn{1}{l|}{\textbf{99.80}} & \multicolumn{1}{l|}{\textbf{99.96}} & \multicolumn{1}{l|}{\textbf{99.98}} & \multicolumn{1}{l|}{\textbf{88.94}} & \textbf{86.87} & \multicolumn{1}{l|}{\textbf{117.72}} & \multicolumn{1}{l|}{\textbf{15.83}} & \multicolumn{1}{l|}{\textbf{151.52}} & \multicolumn{1}{l|}{\textbf{584.60}} & \multicolumn{1}{l|}{\textbf{615.08}} & \textbf{11698.58} & \multicolumn{1}{l|}{\textbf{0.04}} & \multicolumn{1}{l|}{\textbf{0.03}} & \multicolumn{1}{l|}{\textbf{0.06}} & \multicolumn{1}{l|}{\textbf{0.11}} & \multicolumn{1}{l|}{\textbf{76.49}} & \textbf{1767.90} \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoNSW               & \multicolumn{1}{l|}{91.40}          & \multicolumn{1}{l|}{91.30}          & \multicolumn{1}{l|}{99.98}          & \multicolumn{1}{l|}{89.53}          & \multicolumn{1}{l|}{90.48}          & 88.04          & \multicolumn{1}{l|}{1721.73}         & \multicolumn{1}{l|}{212.89}         & \multicolumn{1}{l|}{454.59}          & \multicolumn{1}{l|}{689.47}          & \multicolumn{1}{l|}{1077.06}         & 6205.80           & \multicolumn{1}{l|}{161.95}        & \multicolumn{1}{l|}{20.28}         & \multicolumn{1}{l|}{0.09}          & \multicolumn{1}{l|}{80.61}         & \multicolumn{1}{l|}{113.37}         & 843.11           \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoNSG               & \multicolumn{1}{l|}{99.97}          & \multicolumn{1}{l|}{93.73}          & \multicolumn{1}{l|}{94.33}          & \multicolumn{1}{l|}{99.97}          & \multicolumn{1}{l|}{99.94}          & 94.80          & \multicolumn{1}{l|}{30.62}           & \multicolumn{1}{l|}{302.93}         & \multicolumn{1}{l|}{378.95}          & \multicolumn{1}{l|}{46.18}           & \multicolumn{1}{l|}{48.48}           & 1196.68           & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{20.26}         & \multicolumn{1}{l|}{22.80}         & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.03}           & 65.63            \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoNNDecent          & \multicolumn{1}{l|}{98.26}          & \multicolumn{1}{l|}{98.76}          & \multicolumn{1}{l|}{97.38}          & \multicolumn{1}{l|}{97.93}          & \multicolumn{1}{l|}{98.96}          & 98.94          & \multicolumn{1}{l|}{29.06}           & \multicolumn{1}{l|}{63.56}          & \multicolumn{1}{l|}{54.95}           & \multicolumn{1}{l|}{67.06}           & \multicolumn{1}{l|}{59.79}           & 79.02             & \multicolumn{1}{l|}{0.52}          & \multicolumn{1}{l|}{0.80}          & \multicolumn{1}{l|}{1.48}          & \multicolumn{1}{l|}{1.42}          & \multicolumn{1}{l|}{0.63}           & 0.85             \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoDPG               & \multicolumn{1}{l|}{99.50}          & \multicolumn{1}{l|}{99.43}          & \multicolumn{1}{l|}{99.68}          & \multicolumn{1}{l|}{99.29}          & \multicolumn{1}{l|}{99.39}          & 99.29          & \multicolumn{1}{l|}{442.35}          & \multicolumn{1}{l|}{132.19}         & \multicolumn{1}{l|}{194.15}          & \multicolumn{1}{l|}{165.65}          & \multicolumn{1}{l|}{149.54}          & 334.23            & \multicolumn{1}{l|}{2.20}          & \multicolumn{1}{l|}{0.76}          & \multicolumn{1}{l|}{0.62}          & \multicolumn{1}{l|}{1.18}          & \multicolumn{1}{l|}{0.91}           & 2.39             \\ \hline
\end{tabular}
}
\caption{
Break down the query latency into pending write latency and vector search latency. Full Table of All Datasets. 
}
\label{tab:e2e_bd_full}
\end{minipage}
\begin{minipage}{\textwidth}
     \resizebox{\textwidth}{!}{%
\begin{tabular}{|ll|llllll|llllll|llllll|llllll|llllll}
\cline{1-26}
\multicolumn{2}{|l|}{\multirow{2}{*}{Algorithms}}                                & \multicolumn{6}{l|}{Recall@10}                                                                                                                                                                         & \multicolumn{6}{l|}{Vector Search Latency ($\times 1000 ms$)}                                                                                                                                              & \multicolumn{6}{l|}{Pending Write Latency ($\times 1000 ms$)}                                                                                                                                                        & \multicolumn{6}{l|}{Query Latency ($\times 1000 ms$)}                                                                                                                                                                & \multicolumn{6}{l}{}                                                  \\ \cline{3-26}
\multicolumn{2}{|l|}{}                                                           & \multicolumn{1}{l|}{\Glove}        & \multicolumn{1}{l|}{\SIFT}         & \multicolumn{1}{l|}{\Msong}        & \multicolumn{1}{l|}{\Sun}          & \multicolumn{1}{l|}{\DPR}          & \Trevi        & \multicolumn{1}{l|}{\Glove}        & \multicolumn{1}{l|}{\SIFT}         & \multicolumn{1}{l|}{\Msong}        & \multicolumn{1}{l|}{\Sun}             & \multicolumn{1}{l|}{\DPR}          & \Trevi         & \multicolumn{1}{l|}{\Glove}          & \multicolumn{1}{l|}{\SIFT}           & \multicolumn{1}{l|}{\Msong}          & \multicolumn{1}{l|}{\Sun}             & \multicolumn{1}{l|}{\DPR}             & \Trevi          & \multicolumn{1}{l|}{\Glove}          & \multicolumn{1}{l|}{\SIFT}           & \multicolumn{1}{l|}{\Msong}          & \multicolumn{1}{l|}{\Sun}             & \multicolumn{1}{l|}{\DPR}             & \Trevi          &           &           &           &           &           &           \\ \cline{1-26}
\multicolumn{2}{|l|}{\textbf{\algoBF}}                                           & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \textbf{1.00} & \multicolumn{1}{l|}{\textbf{0.08}} & \multicolumn{1}{l|}{\textbf{0.08}} & \multicolumn{1}{l|}{\textbf{0.15}} & \multicolumn{1}{l|}{\textbf{0.16}}    & \multicolumn{1}{l|}{\textbf{0.24}} & \textbf{1.03}  & \multicolumn{1}{l|}{\textbf{0.35}}   & \multicolumn{1}{l|}{\textbf{0.35}}   & \multicolumn{1}{l|}{\textbf{0.44}}   & \multicolumn{1}{l|}{\textbf{0.54}}    & \multicolumn{1}{l|}{\textbf{0.50}}    & \textbf{1.50}   & \multicolumn{1}{l|}{\textbf{0.43}}   & \multicolumn{1}{l|}{\textbf{0.44}}   & \multicolumn{1}{l|}{\textbf{0.59}}   & \multicolumn{1}{l|}{\textbf{0.70}}    & \multicolumn{1}{l|}{\textbf{0.74}}    & \textbf{2.54}   & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \cline{1-26}
\multicolumn{1}{|l|}{\multirow{5}{*}{Ranging-based}}    & \textbf{\algoLSH}      & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.01}} & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.00}} & \textbf{0.07} & \multicolumn{1}{l|}{\textbf{0.05}} & \multicolumn{1}{l|}{\textbf{0.03}} & \multicolumn{1}{l|}{\textbf{0.06}} & \multicolumn{1}{l|}{\textbf{0.29}}    & \multicolumn{1}{l|}{\textbf{0.02}} & \textbf{12.20} & \multicolumn{1}{l|}{\textbf{0.16}}   & \multicolumn{1}{l|}{\textbf{0.20}}   & \multicolumn{1}{l|}{\textbf{0.17}}   & \multicolumn{1}{l|}{\textbf{0.13}}    & \multicolumn{1}{l|}{\textbf{0.18}}    & \textbf{0.13}   & \multicolumn{1}{l|}{\textbf{0.21}}   & \multicolumn{1}{l|}{\textbf{0.23}}   & \multicolumn{1}{l|}{\textbf{0.23}}   & \multicolumn{1}{l|}{\textbf{0.42}}    & \multicolumn{1}{l|}{\textbf{0.20}}    & \textbf{12.33}  & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \algoFlann             & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{0.00}          & \multicolumn{1}{l|}{0.09}          & \multicolumn{1}{l|}{0.02}          & 0.13          & \multicolumn{1}{l|}{13.66}         & \multicolumn{1}{l|}{14.83}         & \multicolumn{1}{l|}{1.71}          & \multicolumn{1}{l|}{1.84}             & \multicolumn{1}{l|}{37.94}         & 10.02          & \multicolumn{1}{l|}{13.64}           & \multicolumn{1}{l|}{14.81}           & \multicolumn{1}{l|}{1.69}            & \multicolumn{1}{l|}{1.82}             & \multicolumn{1}{l|}{37.89}            & 9.95            & \multicolumn{1}{l|}{0.02}            & \multicolumn{1}{l|}{0.02}            & \multicolumn{1}{l|}{0.02}            & \multicolumn{1}{l|}{0.02}             & \multicolumn{1}{l|}{0.05}             & 0.08            &           &           &           &           &           &           \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \algoPQ                & \multicolumn{1}{l|}{0.12}          & \multicolumn{1}{l|}{0.30}          & \multicolumn{1}{l|}{0.75}          & \multicolumn{1}{l|}{0.53}          & \multicolumn{1}{l|}{0.10}          & 0.53          & \multicolumn{1}{l|}{0.25}          & \multicolumn{1}{l|}{0.25}          & \multicolumn{1}{l|}{0.25}          & \multicolumn{1}{l|}{10.01}            & \multicolumn{1}{l|}{0.25}          & 0.26           & \multicolumn{1}{l|}{2.18}            & \multicolumn{1}{l|}{3.44}            & \multicolumn{1}{l|}{8.58}            & \multicolumn{1}{l|}{363.36}           & \multicolumn{1}{l|}{5.38}             & 21.87           & \multicolumn{1}{l|}{2.44}            & \multicolumn{1}{l|}{3.68}            & \multicolumn{1}{l|}{8.83}            & \multicolumn{1}{l|}{373.37}           & \multicolumn{1}{l|}{5.63}             & 22.14           &           &           &           &           &           &           \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \algoIVFPQ             & \multicolumn{1}{l|}{0.04}          & \multicolumn{1}{l|}{0.23}          & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.33}          & \multicolumn{1}{l|}{0.15}          & 0.42          & \multicolumn{1}{l|}{0.06}          & \multicolumn{1}{l|}{0.06}          & \multicolumn{1}{l|}{0.26}          & \multicolumn{1}{l|}{0.39}             & \multicolumn{1}{l|}{0.33}          & 1.99           & \multicolumn{1}{l|}{4.06}            & \multicolumn{1}{l|}{6.13}            & \multicolumn{1}{l|}{18.68}           & \multicolumn{1}{l|}{5.26}             & \multicolumn{1}{l|}{16.64}            & 20.24           & \multicolumn{1}{l|}{4.11}            & \multicolumn{1}{l|}{6.19}            & \multicolumn{1}{l|}{18.94}           & \multicolumn{1}{l|}{5.66}             & \multicolumn{1}{l|}{16.97}            & 22.22           &           &           &           &           &           &           \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \textbf{\algoOnlinePQ} & \multicolumn{1}{l|}{\textbf{0.12}} & \multicolumn{1}{l|}{\textbf{0.31}} & \multicolumn{1}{l|}{\textbf{0.82}} & \multicolumn{1}{l|}{\textbf{0.52}} & \multicolumn{1}{l|}{\textbf{0.10}} & \textbf{0.52} & \multicolumn{1}{l|}{\textbf{0.25}} & \multicolumn{1}{l|}{\textbf{0.25}} & \multicolumn{1}{l|}{\textbf{0.25}} & \multicolumn{1}{l|}{\textbf{17.04}}   & \multicolumn{1}{l|}{\textbf{0.25}} & \textbf{0.25}  & \multicolumn{1}{l|}{\textbf{2.28}}   & \multicolumn{1}{l|}{\textbf{0.96}}   & \multicolumn{1}{l|}{\textbf{16.61}}  & \multicolumn{1}{l|}{\textbf{382.01}}  & \multicolumn{1}{l|}{\textbf{29.57}}   & \textbf{161.91} & \multicolumn{1}{l|}{\textbf{2.53}}   & \multicolumn{1}{l|}{\textbf{1.21}}   & \multicolumn{1}{l|}{\textbf{16.86}}  & \multicolumn{1}{l|}{\textbf{399.04}}  & \multicolumn{1}{l|}{\textbf{29.81}}   & \textbf{162.16} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \cline{1-26}
\multicolumn{1}{|l|}{\multirow{5}{*}{Navigation-based}} & \textbf{\algoHNSW}     & \multicolumn{1}{l|}{\textbf{0.60}} & \multicolumn{1}{l|}{\textbf{0.90}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{0.99}} & \multicolumn{1}{l|}{\textbf{0.80}} & \textbf{N.A.} & \multicolumn{1}{l|}{\textbf{0.04}} & \multicolumn{1}{l|}{\textbf{0.03}} & \multicolumn{1}{l|}{\textbf{0.05}} & \multicolumn{1}{l|}{\textbf{2362.95}} & \multicolumn{1}{l|}{\textbf{0.13}} & \textbf{N.A.}  & \multicolumn{1}{l|}{\textbf{733.51}} & \multicolumn{1}{l|}{\textbf{178.85}} & \multicolumn{1}{l|}{\textbf{560.26}} & \multicolumn{1}{l|}{\textbf{2048.23}} & \multicolumn{1}{l|}{\textbf{1008.00}} & \textbf{N.A.}   & \multicolumn{1}{l|}{\textbf{733.55}} & \multicolumn{1}{l|}{\textbf{178.88}} & \multicolumn{1}{l|}{\textbf{560.32}} & \multicolumn{1}{l|}{\textbf{4411.18}} & \multicolumn{1}{l|}{\textbf{1008.13}} & \textbf{N.A.}   & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \algoNSW               & \multicolumn{1}{l|}{0.14}          & \multicolumn{1}{l|}{0.55}          & \multicolumn{1}{l|}{0.34}          & \multicolumn{1}{l|}{0.78}          & \multicolumn{1}{l|}{0.52}          & N.A.          & \multicolumn{1}{l|}{0.08}          & \multicolumn{1}{l|}{0.10}          & \multicolumn{1}{l|}{0.09}          & \multicolumn{1}{l|}{662.16}           & \multicolumn{1}{l|}{0.32}          & N.A.           & \multicolumn{1}{l|}{1722.05}         & \multicolumn{1}{l|}{230.58}          & \multicolumn{1}{l|}{2659.85}         & \multicolumn{1}{l|}{727.73}           & \multicolumn{1}{l|}{1349.03}          & N.A.            & \multicolumn{1}{l|}{1722.13}         & \multicolumn{1}{l|}{230.68}          & \multicolumn{1}{l|}{2659.95}         & \multicolumn{1}{l|}{1389.90}          & \multicolumn{1}{l|}{1349.35}          & N.A.            &           &           &           &           &           &           \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \algoNSG               & \multicolumn{1}{l|}{N.A.}          & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{0.00}          & \multicolumn{1}{l|}{0.04}          & \multicolumn{1}{l|}{0.01}          & 0.03          & \multicolumn{1}{l|}{N.A.}          & \multicolumn{1}{l|}{330.88}        & \multicolumn{1}{l|}{388.39}        & \multicolumn{1}{l|}{220.64}           & \multicolumn{1}{l|}{465.39}        & 929.71         & \multicolumn{1}{l|}{N.A.}            & \multicolumn{1}{l|}{330.87}          & \multicolumn{1}{l|}{388.36}          & \multicolumn{1}{l|}{220.62}           & \multicolumn{1}{l|}{465.32}           & 929.59          & \multicolumn{1}{l|}{N.A.}            & \multicolumn{1}{l|}{0.02}            & \multicolumn{1}{l|}{0.03}            & \multicolumn{1}{l|}{0.02}             & \multicolumn{1}{l|}{0.06}             & 0.11            &           &           &           &           &           &           \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \textbf{\algoNNDecent} & \multicolumn{1}{l|}{\textbf{0.01}} & \multicolumn{1}{l|}{\textbf{0.12}} & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.23}} & \multicolumn{1}{l|}{\textbf{0.17}} & \textbf{0.46} & \multicolumn{1}{l|}{\textbf{0.60}} & \multicolumn{1}{l|}{\textbf{0.82}} & \multicolumn{1}{l|}{\textbf{0.76}} & \multicolumn{1}{l|}{\textbf{1.31}}    & \multicolumn{1}{l|}{\textbf{0.78}} & \textbf{1.13}  & \multicolumn{1}{l|}{\textbf{266.65}} & \multicolumn{1}{l|}{\textbf{590.58}} & \multicolumn{1}{l|}{\textbf{389.62}} & \multicolumn{1}{l|}{\textbf{339.08}}  & \multicolumn{1}{l|}{\textbf{555.88}}  & \textbf{733.62} & \multicolumn{1}{l|}{\textbf{267.26}} & \multicolumn{1}{l|}{\textbf{591.39}} & \multicolumn{1}{l|}{\textbf{390.37}} & \multicolumn{1}{l|}{\textbf{340.39}}  & \multicolumn{1}{l|}{\textbf{556.66}}  & \textbf{734.74} &           &           &           &           &           &           \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \algoDPG               & \multicolumn{1}{l|}{0.08}          & \multicolumn{1}{l|}{0.33}          & \multicolumn{1}{l|}{0.06}          & \multicolumn{1}{l|}{0.30}          & \multicolumn{1}{l|}{0.31}          & 0.48          & \multicolumn{1}{l|}{1.66}          & \multicolumn{1}{l|}{1.02}          & \multicolumn{1}{l|}{2.23}          & \multicolumn{1}{l|}{1.22}             & \multicolumn{1}{l|}{1.26}          & 3.27           & \multicolumn{1}{l|}{7637.47}         & \multicolumn{1}{l|}{1133.86}         & \multicolumn{1}{l|}{5007.04}         & \multicolumn{1}{l|}{905.62}           & \multicolumn{1}{l|}{1334.21}          & 4304.74         & \multicolumn{1}{l|}{7639.13}         & \multicolumn{1}{l|}{1134.88}         & \multicolumn{1}{l|}{5009.27}         & \multicolumn{1}{l|}{906.83}           & \multicolumn{1}{l|}{1335.47}          & 4308.02         &           &           &           &           &           &           \\ \cline{1-26}
\end{tabular}
}
\caption{Results of cross-validation. N.A. means that the evaluation of certain algorithms and certain datasets exceeds 4h wall time, and therefore unable to get further results. We observe that all of the N.A. is caused by the large overhead of pending writings.}
\label{tab:e2e_cross}
\end{minipage}
\end{sidewaystable}






==> Evaluations/Environ.tex <==
\subsection{Sensitivity to the Online Environment}
In this evaluation, we investigate how the online environment itself will affect AKNN algorithms. Specifically, we focus on both the arrival rate of input vectors and the distribution shift on its content.
\begin{quote}
    Observation \themyvar.
    {A higher event rate generally makes AKNN more prone to low recall and high query latency, it further leads to fluctuation of query latency in navigation-based AKNN.}
\end{quote}
\stepcounter{myvar}
\begin{figure}[t]
\begin{minipage}[a]{\textwidth} 
\centering
         \begin{minipage} [b] {0.70\textwidth}
        \begin{minipage}[c]{0.57\textwidth}
        \centering
        \subfigure[Query Recall]{
            \includegraphics[width=0.99\textwidth]{figures/scanIPEventRate_recall_feedMode.pdf}
            \label{fig:rate_recall}
        }
    \end{minipage}
    \begin{minipage}[c]{0.41\textwidth}
        \subfigure[Query Latency.]{
            \includegraphics[width=0.99\textwidth]{figures/scanIPEventRate_lat_instant_search.pdf}
            \label{fig:rate_lat}
        }
    \end{minipage}     
    \caption{Tuning event rate from $20$ to $5000$, the unit is $rows/s$. \algoNNDecent is N.A. to show as it constantly exceeds the wall time.}
        \label{fig:event_rate}
    \end{minipage}
    
\end{minipage}
\end{figure}
We first investigate the impacts of the event rate. We utilize the \DPR data while tuning the data generation speed at the data source from $100 rows/s \sim xx rows/s$. The resulting query latency and recall are shown in Figure~\ref{fig:event_rate}. 
{In general, once the event rate exceeds the ingestion capacity of AKNN, e.g..., about 20 for \algoHNSW, it leads to both higher query latency and lower recall as more data is dropped.} On the contrary, although some AKNN like \algoLSH is lightweight and keeps up the data source even at 5000 $rows/s$ speed, its recall is inherently too low to be practically adapted. We further observe that navigation-based AKNN (i.e., \algoHNSW,\algoNSW,\algoNSG) leads to a larger fluctuation of query latency than ranging-based AKNN, i.e., up to $\times 10$ more than \algoLSH or \algoIVFPQ. This is because the data ingestion of navigation-based AKNN requires an iterative scan and comparison within the proximity graph. Compared with the straight-forward data flow of ranging-based AKNN (Section~\ref{sec:bg}), this is more costly and more sensitive to the unmatched data arrival and data ingestion.

%

We next examine the impacts of distribution shifts, focusing specifically on the effects of occurrence position and general intensity of distribution shifts, which we analyze individually. Our evaluations are conducted using \Wte.
\begin{quote}
    Observation \themyvar.
    {Most AKNNs are challenged by distribution shifts, no matter where the shift starts to occur. On the contrary, navigation-based \algoHNSW is more resilient than others.}
\end{quote}
\stepcounter{myvar}
\begin{figure}[t]
\begin{minipage}[a]{\textwidth} 

         \begin{minipage} [b] {0.70\textwidth}
        \begin{minipage}[c]{0.57\textwidth}
        \centering
        \subfigure[Query Recall]{
            \includegraphics[width=0.99\textwidth]{figures/scanIPConceptDriftTopic_recall.pdf}
            \label{fig:cd_recall}
        }
    \end{minipage}
    \begin{minipage}[c]{0.41\textwidth}
        \subfigure[Query Latency.]{
            \includegraphics[width=0.99\textwidth]{figures/scanIPConceptDriftTopic_lat_instant.pdf}
            \label{fig:cd_lat}
        }
    \end{minipage}     
    \caption{Tuning the occurrence position of distribution shift. The Red dashed line indicates where the distribution shift occurs exactly at the same place as the beginning of online ingested data. \algoNNDecent is N.A. to show as it still exceeds the wall time. --\xianzhi{some results are strange and running confirmations.}}
        \label{fig:cd_pos}
    \end{minipage}
    \begin{minipage}[b]{0.29\textwidth}
        \includegraphics*[width=0.99\textwidth]{figures/scanIPConceptDriftHotSpot_recall.pdf}
        \caption{Tuning the intensity of distribution shift. A larger replacing probability indicates higher intensity.}
    \label{fig:cd_intensity}
    \end{minipage}    
\end{minipage}
\end{figure}

To begin, we manipulate the occurrence position of distribution shifts. Using the synthetic dataset \Wte, with all other settings kept as default, we initiate our experimentation by generating vector embeddings from USA aircraft and subsequently transitioning to vector embeddings of USSR land vehicles. The starting position of the USSR land vehicles' embeddings varies from 1000 to 90000, indicating varying occurrence positions of distribution shift. Notably, if the shift occurs prior to 50000, the initial phase of this transition is already accounted for during the offline setup of loading initial data (see Section~\ref{subsec:general_setup}). The resulting metrics for query recall and latency are presented in Figure~\ref{fig:cd_pos}.
%
Overall, \algoHNSW demonstrates the highest resilience to the distribution shift, maintaining a recall rate of over 0.4. However, it experiences slight fluctuations in both latency and recall. This variability can be attributed to the significant dissimilarity between the embedding vectors of USSR land vehicles and those of USA aircraft. \algoHNSW may opt to either create a new graph cluster for the shifted data or endeavor to place it in the most appropriate location within the existing structure. While the former approach is relatively lightweight and accurate, the latter necessitates traversing through relatively irrelevant graph vertices, incurring higher costs and potential inaccuracies. The tension between these choices is the primary driver behind the observed fluctuations.
%
On the contrary, all of the other evaluated AKNN, fail to achieve a recall rate above 0.1. 
%
\xianzhi{Moreover, a ranging-based AKNN, i.e.,  \algoIVFPQ, involve a huge fluctuation when the distribution shift is introduced near the beginning of online ingested data. This is due to 
their strong assumption on known and unchanged data distribution and their pre-trained cluster centroids are especially prone to the changes. 
 Compared with \algoIVFPQ, such fluctuation effect is further amplified by the hierarchical design involved.
}
%
Furthermore, despite its intentional efforts to adapt to changing conditions, \algoOnlinePQ's simplistic update rule proves insufficient, leading to suboptimal performance (i.e., even less compatible than \algoPQ). It struggles to reconcile the original USA aircraft data with the new USSR land vehicle data effectively. Consequently, it settles into an ineffective intermediate state where neither the old nor the new data can be accurately ingested or indexed.

\begin{quote}
    Observation \themyvar.
    {\algoHNSW is also resilient to relatively intensive distribution shifts, while none of the other AKNN handles it well.}
\end{quote}
\stepcounter{myvar}

We then explore variations in the general intensity of distribution shifts. Specifically, we construct the entire sentence collection using nouns related to USA aircraft. Subsequently, we induce a distribution shift at 50000 by randomly replacing the subject noun with a specific USSR land vehicle, namely ``T-34-85". The resulting sentence, contaminated by this shift, is then used to generate embeddings.
%
This process emulates real-world scenarios where a sudden emergence of a prominent topic occurs, represented here by ``T-34-85". The intensity of the shift is further adjusted by varying the probability of word contamination, ranging from 0.05 to 0.8. The resulting changes in query recall are depicted in Figure~\ref{fig:cd_intensity}. The query latency is omitted as it's similar to the case of evaluating \DPR dataset in Table~\ref{tab:e2e_ip}, and there are only up to $5\%$ fluctuations for each algorithm.
%
Overall, all AKNN methods except \algoHNSW consistently exhibit low recall and high latency, with recall consistently below 0.4. In contrast, \algoHNSW demonstrates increasing recall as the intensity of the shift grows. This can be attributed to its robust heuristics and hierarchical structure. Specifically, \algoHNSW automatically groups the distribution shift data related to the ``T-34-85" topic in its proxy graph, enhancing the possibility of retrieving relevant data without relying on strong assumptions. Additionally, unlike \algoNSW, the hierarchical design of \algoHNSW helps control the scale of each group, thereby reducing the inclusion of irrelevant query results and further enhancing accuracy.
%
If the significant overhead associated with pending writing  (i.e., as discussed in Section~\ref{subsec:overall}) can be effectively addressed, \algoHNSW could emerge as the optimal choice for ingesting online data even amidst distribution shifts.

==> Evaluations/Other.tex <==

\subsection{Other Sensitive Factors under Online Ingestion Settings}
\begin{figure}[t]
\begin{minipage}[a]{\textwidth} 
\centering
         \begin{minipage} [b] {0.70\textwidth}
        \begin{minipage}[c]{0.57\textwidth}
        \centering
        \subfigure[Query Recall]{
            \includegraphics[width=0.99\textwidth]{figures/scanIPEventRateFaissHalf_recall_feedMode.pdf}
            \label{fig:batch_recall}
        }
    \end{minipage}
    \begin{minipage}[c]{0.41\textwidth}
        \subfigure[Query Latency.]{
            \includegraphics[width=0.99\textwidth]{figures/scanIPEventRateFaissHalf_lat_instant_search.pdf}
            \label{fig:batch_lat}
        }
    \end{minipage}     
    \caption{Tuning the size of micro-batches from 200 to 50000. }
        \label{fig:batch}
    \end{minipage}
    
\end{minipage}
\end{figure}

In this evaluation, we investigate how the other common concerns of AKNN turn out to be under our new setting of online ingestion. Specifically, we revisit the impacts of micron batch agglomeration, vector dimension, and vector volumes.
\begin{quote}
    Observation \themyvar.
    {The size of agglomeration micro-batches has a significant and complicated impact on both query recall and latency, and there is no universal optimal setting for all evaluated AKNN.}
\end{quote}
\stepcounter{myvar}

The data science community widely recognizes the utility of micro-batching for consolidating data to serve various objectives. On one side, segmenting extensive datasets into smaller micro-batches enables more frequent updates to machine learning model parameters, facilitating quicker convergence~\cite{huang2019gpipe,yuan2022decentralized}. Conversely, lazily agglomerating more data instead of a relatively eager stream processing can enhance the throughput of online database systems~\cite{zhang2021parallelizing}. Drawing inspiration from existing research, we experimented with adjusting the micro-batch size for AKNN data ingestion from 200 to 50,000 and observed the effects on query latency. The resulting query recall and latency are demonstrated in Figure~\ref{fig:batch}.

It becomes evident that there isn't a universally ideal batch size suitable for all AKNN algorithms; selecting an optimal size necessitates a nuanced, algorithm-specific decision. For inherently more complex algorithms that process vector points individually, such as 
\algoHNSW, \algoNSW, and \algoNSG, opting for a larger batch size results in less efficient use of processing time, which in turn, increases query latency (Figure~\ref{fig:batch_lat}). The decision becomes more intricate for other algorithms, where the benefits of agglomeration and the drawbacks of under-utilization occur concurrently. This scenario demands a balanced approach, making a moderate batch size the preferable choice. An example of this can be seen with 
\algoLSH
\algoLSH, where a specific moderate batch size emerges as the most efficient option, embodying the delicate equilibrium between aggregation benefits and processor utilization efficiency.


We observe that batch size significantly influences query recall, as illustrated in~\ref{fig:batch_recall}. This effect is primarily due to its impact on ingestion efficiency, which is further exacerbated by data droppings.
%
Interestingly, even \algoBF, typically expected to perform exact searches, exhibits inaccuracies when the batch size is small (e.g., 200) and data dropping occurs.
%
Conversely, larger batch sizes reduce the time required to divide ingested data and decrease the static overhead associated with data ingestion, thereby increasing the completeness of ingested data when facing the risk of dropping data. Consequently, this usually results in enhanced recall for all algorithms evaluated.

\begin{quote}
    Observation \themyvar.
    {The notorious ``curse of dimension~\cite{}'' is even more complicated in online ingestion, highlighting the importance of improving ingestion efficiency.}
\end{quote}
\stepcounter{myvar}
Data scalability to vector dimension remains a key concern for AKNN as highlighted in existing studies~\cite{li2019approximate}. We explored this aspect in online ingestion using \Random, adjusting the data dimension from $64$ to $4096$, while maintaining other settings at their default values. We observed two major insights:

First, consistent with static data scenarios~\cite{li2019approximate}, navigation-based AKNN such as \algoHNSW generally outperforms range-based AKNN (e.g., \algoIVFPQ) in terms of query recall (Figure~\ref{fig:dim_recall}). This superiority stems from their ability to better preserve the relationships among ingested data and involve fewer assumptions. However, this robust design comes at the cost of a larger memory footprint, which has led to out-of-memory issues during our evaluations.
%
Second, in contrast to common beliefs~\cite{li2019approximate,malkov2018efficient}, most of the AKNN algorithms we tested, with the exception of \algoLSH, are more susceptible to the 
the ``curse of dimension'' than \algoBF, and they demonstrate more significant growth in query latency with dimensions increases (Figure~\ref{fig:dim_lat}). This finding contradicts the expectation that AKNN algorithms are optimized for vector search with minimal performance degradation as dimensions increase. Notably, while most AKNN designs aim to reduce overhead and maintain resilience to increasing dimensions in the vector search phase~\cite{jegou2010product,malkov2018efficient}, their ingestion processes do not exhibit the same efficiency, resulting in higher overall query latency. This reaffirms that there is an over-optimization in vector search capabilities at the expense of ingestion performance, highlighting a critical area for further improvement in AKNN systems.

\begin{figure}[t]
\begin{minipage}[a]{\textwidth} 
\centering
         \begin{minipage} [b] {0.70\textwidth}
        \begin{minipage}[c]{0.57\textwidth}
        \centering
        \subfigure[Query Recall]{
            \includegraphics[width=0.99\textwidth]{figures/scanIPDimensions_recall_feedMode.pdf}
            \label{fig:dim_recall}
        }
    \end{minipage}
    \begin{minipage}[c]{0.41\textwidth}
        \subfigure[Query Latency.]{
            \includegraphics[width=0.99\textwidth]{figures/scanIPDimensions_lat_instant_search.pdf}
            \label{fig:dim_lat}
        }
    \end{minipage}     
    \caption{Revisit the ``curse of dimension'' under online ingestion. \algoHNSW and \algoNSW run out of memory under 4096-D case.}
        \label{fig:dim}
    \end{minipage}
    
\end{minipage}
\end{figure}


\begin{quote}
    Observation \themyvar.
    {The vector volume is also impactful under online ingestion, and it requires more careful design under the possibility of dropping data.}
\end{quote}
\stepcounter{myvar}
\begin{figure}[t]
\begin{minipage}[a]{\textwidth} 
\centering
         \begin{minipage} [b] {0.70\textwidth}
        \begin{minipage}[c]{0.57\textwidth}
        \centering
        \subfigure[Query Recall]{
            \includegraphics[width=0.99\textwidth]{figures/scanIPVecVolume_recall_feedMode.pdf}
            \label{fig:vecVol_recall}
        }
    \end{minipage}
    \begin{minipage}[c]{0.41\textwidth}
        \subfigure[Query Latency.]{
            \includegraphics[width=0.99\textwidth]{figures/scanIPVecVolume_lat_instant_search.pdf}
            \label{fig:vecVol_lat}
        }
    \end{minipage}     
    \caption{Tuning the vector volume from $60K \sim 5M$. \xianzhi{--Rember to redo some strange data points.}}
        \label{fig:vecVol}
    \end{minipage}
    
\end{minipage}
\end{figure}

Data scalability to vector volume is a significant concern for Approximate AKNN as identified in previous studies~\cite{li2019approximate}. To explore this under online ingestion conditions, we employed \Random with vector volumes adjusted from $60K$ to $5M$, while maintaining default settings for other parameters. Notably, the beginning $50K$ vectors were loaded during the offline construction phase prior to online ingestion. The impact of these changes on query recall and latency is shown in~\ref{fig:vecVol}. Our observations are twofold:
%
First, as anticipated, most AKNN algorithms exhibit an increase in query latency as vector volume increases (Figure~\ref{fig:vecVol_lat}). Interestingly, the rate of increase in query latency for some algorithms, such as \algoOnlinePQ, is less pronounced compared to \algoBF. This observation is consistent with expectations set by previous research~\cite{li2019approximate,xu2018online}.
%
Second, in a more complex scenario than the static data case~\cite{li2019approximate,xu2018online,malkov2018efficient}, escalating vector volumes introduce new accuracy challenges for AKNN (Figure~\ref{fig:vecVol_recall}). For instance, while \algoHNSW was the most accurate in previous evaluations, its accuracy diminishes below that of \algoLSH when the volume reaches $500K$. This deviation is in stark contrast to findings from~\cite{malkov2018efficient}, where \algoHNSW consistently maintained high recall across varying data volumes. The decrease in accuracy can be attributed to the low ingestion efficiency of \algoHNSW; as vector volume increases, more data is dropped, leading to less accurate vector searches.




==> Evaluations/Overall.tex <==

\subsection{Overall Results}
\label{subsec:overall}
We first investigate how different AKNN performs under the real-world datasets, concerning both query latency and query recall, as summarized 
in Tables~\ref{tab:e2e_ip} for both inner product and L2 distance, respectively. 
\begin{quote}
    Observation \themyvar. Contrary to common belief~\cite{li2019approximate}, \xianzhi{nearly none of the evaluated AKNN outperforms the brutal force under the online ingestion cases. 
    }
\end{quote}
\stepcounter{myvar}
\begin{table}[]
\centering
 \resizebox{0.99\textwidth}{!}{%
\begin{tabular}{|ll|llllllllllll|llllllllllll|}
\hline
\multicolumn{2}{|l|}{\multirow{3}{*}{Algorithms}}                                & \multicolumn{12}{l|}{Inner Product}                                                                                                                                                                                                                                                                                                                                                                                                               & \multicolumn{12}{l|}{L2 Distance}                                                                                                                                                                                                                                                                                                                                                                                                                \\ \cline{3-26} 
\multicolumn{2}{|l|}{}                                                           & \multicolumn{6}{l|}{Recall@10}                                                                                                                                                                                              & \multicolumn{6}{l|}{Query Latency ($\times 1000 ms$)}                                                                                                                                                               & \multicolumn{6}{l|}{Recall@10}                                                                                                                                                                                              & \multicolumn{6}{l|}{Query Latency ($\times 1000 ms$)}                                                                                                                                                              \\ \cline{3-26} 
\multicolumn{2}{|l|}{}                                                           & \multicolumn{1}{l|}{\Glove}        & \multicolumn{1}{l|}{\SIFT}         & \multicolumn{1}{l|}{\Msong}        & \multicolumn{1}{l|}{\Sun}          & \multicolumn{1}{l|}{\DPR}          & \multicolumn{1}{l|}{\Trevi}        & \multicolumn{1}{l|}{\Glove}          & \multicolumn{1}{l|}{\SIFT}          & \multicolumn{1}{l|}{\Msong}          & \multicolumn{1}{l|}{\Sun}            & \multicolumn{1}{l|}{\DPR}            & \Trevi            & \multicolumn{1}{l|}{\Glove}        & \multicolumn{1}{l|}{\SIFT}         & \multicolumn{1}{l|}{\Msong}        & \multicolumn{1}{l|}{\Sun}          & \multicolumn{1}{l|}{\DPR}          & \multicolumn{1}{l|}{\Trevi}        & \multicolumn{1}{l|}{\Glove}          & \multicolumn{1}{l|}{\SIFT}          & \multicolumn{1}{l|}{\Msong}          & \multicolumn{1}{l|}{\Sun}            & \multicolumn{1}{l|}{\DPR}            & \Trevi           \\ \hline
\multicolumn{2}{|l|}{\textbf{\algoBF}}                                           & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{0.43}}   & \multicolumn{1}{l|}{\textbf{0.44}}  & \multicolumn{1}{l|}{\textbf{0.60}}   & \multicolumn{1}{l|}{\textbf{0.69}}   & \multicolumn{1}{l|}{\textbf{0.76}}   & \textbf{2.53}     & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{0.67}}   & \multicolumn{1}{l|}{\textbf{0.68}}  & \multicolumn{1}{l|}{\textbf{0.98}}   & \multicolumn{1}{l|}{\textbf{0.98}}   & \multicolumn{1}{l|}{\textbf{1.13}}   & \textbf{4.09}    \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{Ranging-based}}    & \textbf{\algoLSH}      & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.01}} & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.07}} & \multicolumn{1}{l|}{\textbf{0.17}}   & \multicolumn{1}{l|}{\textbf{0.22}}  & \multicolumn{1}{l|}{\textbf{0.23}}   & \multicolumn{1}{l|}{\textbf{0.42}}   & \multicolumn{1}{l|}{\textbf{0.19}}   & \textbf{11.96}    & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.01}} & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.07}} & \multicolumn{1}{l|}{\textbf{0.18}}   & \multicolumn{1}{l|}{\textbf{0.23}}  & \multicolumn{1}{l|}{\textbf{0.23}}   & \multicolumn{1}{l|}{\textbf{0.48}}   & \multicolumn{1}{l|}{\textbf{0.19}}   & \textbf{11.99}   \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                                  & \algoPQ                & \multicolumn{1}{l|}{0.09}          & \multicolumn{1}{l|}{0.22}          & \multicolumn{1}{l|}{0.50}          & \multicolumn{1}{l|}{0.42}          & \multicolumn{1}{l|}{0.09}          & \multicolumn{1}{l|}{0.38}          & \multicolumn{1}{l|}{354.43}          & \multicolumn{1}{l|}{351.58}         & \multicolumn{1}{l|}{358.40}          & \multicolumn{1}{l|}{363.92}          & \multicolumn{1}{l|}{361.51}          & 414.77            & \multicolumn{1}{l|}{0.14}          & \multicolumn{1}{l|}{0.36}          & \multicolumn{1}{l|}{0.61}          & \multicolumn{1}{l|}{0.44}          & \multicolumn{1}{l|}{0.10}          & \multicolumn{1}{l|}{0.40}          & \multicolumn{1}{l|}{1.57}            & \multicolumn{1}{l|}{1.52}           & \multicolumn{1}{l|}{2.35}            & \multicolumn{1}{l|}{362.87}          & \multicolumn{1}{l|}{361.64}          & 2.58             \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                                  & \algoIVFPQ             & \multicolumn{1}{l|}{0.03}          & \multicolumn{1}{l|}{0.23}          & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{0.33}          & \multicolumn{1}{l|}{0.11}          & \multicolumn{1}{l|}{0.28}          & \multicolumn{1}{l|}{393.40}          & \multicolumn{1}{l|}{2.11}           & \multicolumn{1}{l|}{400.55}          & \multicolumn{1}{l|}{2.85}            & \multicolumn{1}{l|}{409.62}          & 504.46            & \multicolumn{1}{l|}{0.03}          & \multicolumn{1}{l|}{0.13}          & \multicolumn{1}{l|}{0.31}          & \multicolumn{1}{l|}{0.30}          & \multicolumn{1}{l|}{0.12}          & \multicolumn{1}{l|}{0.11}          & \multicolumn{1}{l|}{1.44}            & \multicolumn{1}{l|}{405.34}         & \multicolumn{1}{l|}{415.41}          & \multicolumn{1}{l|}{422.30}          & \multicolumn{1}{l|}{425.20}          & 530.54           \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                                  & \textbf{\algoOnlinePQ} & \multicolumn{1}{l|}{\textbf{0.12}} & \multicolumn{1}{l|}{\textbf{0.31}} & \multicolumn{1}{l|}{\textbf{0.78}} & \multicolumn{1}{l|}{\textbf{0.43}} & \multicolumn{1}{l|}{\textbf{0.09}} & \multicolumn{1}{l|}{\textbf{0.38}} & \multicolumn{1}{l|}{\textbf{1.60}}   & \multicolumn{1}{l|}{\textbf{1.20}}  & \multicolumn{1}{l|}{\textbf{3.36}}   & \multicolumn{1}{l|}{\textbf{384.48}} & \multicolumn{1}{l|}{\textbf{395.55}} & \textbf{19.20}    & \multicolumn{1}{l|}{\textbf{0.14}} & \multicolumn{1}{l|}{\textbf{0.37}} & \multicolumn{1}{l|}{\textbf{0.46}} & \multicolumn{1}{l|}{\textbf{0.44}} & \multicolumn{1}{l|}{\textbf{0.10}} & \multicolumn{1}{l|}{\textbf{0.38}} & \multicolumn{1}{l|}{\textbf{1.63}}   & \multicolumn{1}{l|}{\textbf{1.21}}  & \multicolumn{1}{l|}{\textbf{374.20}} & \multicolumn{1}{l|}{\textbf{384.45}} & \multicolumn{1}{l|}{\textbf{4.90}}   & \textbf{605.60}  \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{Navigation-based}} & \textbf{\algoHNSW}     & \multicolumn{1}{l|}{\textbf{0.39}} & \multicolumn{1}{l|}{\textbf{0.54}} & \multicolumn{1}{l|}{\textbf{0.61}} & \multicolumn{1}{l|}{\textbf{0.77}} & \multicolumn{1}{l|}{\textbf{0.46}} & \multicolumn{1}{l|}{\textbf{0.51}} & \multicolumn{1}{l|}{\textbf{117.76}} & \multicolumn{1}{l|}{\textbf{15.86}} & \multicolumn{1}{l|}{\textbf{151.58}} & \multicolumn{1}{l|}{\textbf{584.71}} & \multicolumn{1}{l|}{\textbf{691.58}} & \textbf{13466.48} & \multicolumn{1}{l|}{\textbf{0.15}} & \multicolumn{1}{l|}{\textbf{0.47}} & \multicolumn{1}{l|}{\textbf{0.60}} & \multicolumn{1}{l|}{\textbf{0.68}} & \multicolumn{1}{l|}{\textbf{0.42}} & \multicolumn{1}{l|}{\textbf{0.51}} & \multicolumn{1}{l|}{\textbf{144.37}} & \multicolumn{1}{l|}{\textbf{37.66}} & \multicolumn{1}{l|}{\textbf{334.64}} & \multicolumn{1}{l|}{\textbf{107.47}} & \multicolumn{1}{l|}{\textbf{877.98}} & \textbf{1454.51} \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                                  & \algoNSW               & \multicolumn{1}{l|}{0.10}          & \multicolumn{1}{l|}{0.35}          & \multicolumn{1}{l|}{0.28}          & \multicolumn{1}{l|}{0.63}          & \multicolumn{1}{l|}{0.33}          & \multicolumn{1}{l|}{0.51}          & \multicolumn{1}{l|}{1883.68}         & \multicolumn{1}{l|}{233.17}         & \multicolumn{1}{l|}{454.67}          & \multicolumn{1}{l|}{770.08}          & \multicolumn{1}{l|}{1190.43}         & 7048.91           & \multicolumn{1}{l|}{0.12}          & \multicolumn{1}{l|}{0.45}          & \multicolumn{1}{l|}{0.58}          & \multicolumn{1}{l|}{0.64}          & \multicolumn{1}{l|}{0.39}          & \multicolumn{1}{l|}{0.51}          & \multicolumn{1}{l|}{1887.25}         & \multicolumn{1}{l|}{233.03}         & \multicolumn{1}{l|}{456.04}          & \multicolumn{1}{l|}{771.52}          & \multicolumn{1}{l|}{1191.62}         & 1674.74          \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                                  & \algoNSG               & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{0.00}          & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{0.03}          & \multicolumn{1}{l|}{30.62}           & \multicolumn{1}{l|}{323.19}         & \multicolumn{1}{l|}{401.75}          & \multicolumn{1}{l|}{46.20}           & \multicolumn{1}{l|}{48.51}           & 1262.32           & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{0.00}          & \multicolumn{1}{l|}{0.03}          & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{0.03}          & \multicolumn{1}{l|}{30.68}           & \multicolumn{1}{l|}{30.44}          & \multicolumn{1}{l|}{402.25}          & \multicolumn{1}{l|}{46.29}           & \multicolumn{1}{l|}{48.35}           & 1263.94          \\ \cline{2-26} 
\multicolumn{1}{|l|}{}                                  & \textbf{\algoNNDecent} & \multicolumn{6}{l|}{\textbf{N.A.}}                                                                                                                                                                                          & \multicolumn{6}{l|}{\textbf{N.A.}}                                                                                                                                                                                & \multicolumn{6}{l|}{\textbf{N.A.}}                                                                                                                                                                                          & \multicolumn{6}{l|}{\textbf{N.A.}}                                                                                                                                                                               \\ \hline
\end{tabular}
}
\caption{Overall Comparison under Inner Product and L2 Distance. The query latency of \algoNNDecent exceeds 4 hours of wall time and we can't calculate its recall.}
\label{tab:e2e_ip}
\end{table}

When we focus on the inner product, we observe that only \algoLSH outperforms \algoBF in terms of query latency for some datasets (e.g., $75\%$ less in \DPR), but it is too inaccurate to be applied and the recall is at most 0.01. \algoOnlinePQ and \algoHNSW are the most accurate among ranging-based and navigation-based AKNN, respectively, with recall yields up to 0.7. Nevertheless, their query latency is significantly larger than the \algoBF , i.e., $908\times$ more in \DPR. 
\xianzhi{The results of \algoNNDecent are even more surprising. Although it is considered a light-weight navigation-based AKNN in static data cases~\cite{}, it leads to the highest query latency among all. We observe that this is because \algoNNDecent involves a strong assumption of known \xianzhi{xxx properties and fixed data amount}. For each update raised by online ingestion, it has to rebuild the proxy graph from scratch.}

The comparison under L2 distance is similar, and none of the evaluated AKNN outperforms \algoBF. Besides, there are two slight differences from inner production cases to be noted. First, \algoOnlinePQ is less accurate than \algoPQ in some datasets like \Msong and \Trevi. This is because it involves linear incremental updates, which are sometimes not fully aligned with the square sum specified in L2 distance semantics. Second, \algoNSW is much more accurate 
under L2 distance than inner product for some datasets like \Msong. i.e., 0.58 v.s., 0.28. On the contrary, \algoHNSW, which introduces a hierarchical design for optimizations, is generally more stable and demonstrates fewer recall differences under different distance metrics.



%\xianzhi{--Table of IP and L2 E2E}
\begin{quote}
    Observation \themyvar.
    The impacts of pending writings are dominant to the failure of evaluated AKNN.
\end{quote}
\stepcounter{myvar}
\begin{table}[]
\centering
 \resizebox{0.99\textwidth}{!}{%
\begin{tabular}{|ll|llllll|llllll|llllll|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{Algorithms}}                                & \multicolumn{6}{l|}{Propotion of Pending Write Latency (\%)}                                                                                                                                                 & \multicolumn{6}{l|}{Pending Write Latency ($\times 1000 ms$)}                                                                                                                                                       & \multicolumn{6}{l|}{Vector Search Latency ($\times 1000 ms$)}                                                                                                                                              \\ \cline{3-20} 
\multicolumn{2}{|l|}{}                                                           & \multicolumn{1}{l|}{\Glove}         & \multicolumn{1}{l|}{\SIFT}          & \multicolumn{1}{l|}{\Msong}         & \multicolumn{1}{l|}{\Sun}           & \multicolumn{1}{l|}{\DPR}           & \Trevi         & \multicolumn{1}{l|}{\Glove}          & \multicolumn{1}{l|}{\SIFT}          & \multicolumn{1}{l|}{\Msong}          & \multicolumn{1}{l|}{\Sun}            & \multicolumn{1}{l|}{\DPR}            & \Trevi            & \multicolumn{1}{l|}{\Glove}        & \multicolumn{1}{l|}{\SIFT}         & \multicolumn{1}{l|}{\Msong}        & \multicolumn{1}{l|}{\Sun}          & \multicolumn{1}{l|}{\DPR}           & \Trevi           \\ \hline
\multicolumn{2}{|l|}{\textbf{\algoBF}}                                           & \multicolumn{1}{l|}{\textbf{83.29}} & \multicolumn{1}{l|}{\textbf{79.50}} & \multicolumn{1}{l|}{\textbf{73.13}} & \multicolumn{1}{l|}{\textbf{78.20}} & \multicolumn{1}{l|}{\textbf{63.32}} & \textbf{59.96} & \multicolumn{1}{l|}{\textbf{0.36}}   & \multicolumn{1}{l|}{\textbf{0.35}}  & \multicolumn{1}{l|}{\textbf{0.44}}   & \multicolumn{1}{l|}{\textbf{0.54}}   & \multicolumn{1}{l|}{\textbf{0.48}}   & \textbf{1.51}     & \multicolumn{1}{l|}{\textbf{0.07}} & \multicolumn{1}{l|}{\textbf{0.09}} & \multicolumn{1}{l|}{\textbf{0.16}} & \multicolumn{1}{l|}{\textbf{0.15}} & \multicolumn{1}{l|}{\textbf{0.28}}  & \textbf{1.01}    \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{Ranging-based}}    & \algoLSH               & \multicolumn{1}{l|}{91.08}          & \multicolumn{1}{l|}{86.38}          & \multicolumn{1}{l|}{74.99}          & \multicolumn{1}{l|}{30.49}          & \multicolumn{1}{l|}{89.10}          & 1.11           & \multicolumn{1}{l|}{0.16}            & \multicolumn{1}{l|}{0.19}           & \multicolumn{1}{l|}{0.17}            & \multicolumn{1}{l|}{0.13}            & \multicolumn{1}{l|}{0.17}            & 0.13              & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.03}          & \multicolumn{1}{l|}{0.06}          & \multicolumn{1}{l|}{0.29}          & \multicolumn{1}{l|}{0.02}           & 11.83            \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoPQ                & \multicolumn{1}{l|}{99.67}          & \multicolumn{1}{l|}{99.62}          & \multicolumn{1}{l|}{99.55}          & \multicolumn{1}{l|}{99.61}          & \multicolumn{1}{l|}{99.61}          & 99.53          & \multicolumn{1}{l|}{353.26}          & \multicolumn{1}{l|}{350.25}         & \multicolumn{1}{l|}{356.80}          & \multicolumn{1}{l|}{362.51}          & \multicolumn{1}{l|}{360.10}          & 412.80            & \multicolumn{1}{l|}{1.17}          & \multicolumn{1}{l|}{1.33}          & \multicolumn{1}{l|}{1.60}          & \multicolumn{1}{l|}{1.41}          & \multicolumn{1}{l|}{1.40}           & 1.97             \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoIVFPQ             & \multicolumn{1}{l|}{99.67}          & \multicolumn{1}{l|}{97.20}          & \multicolumn{1}{l|}{99.52}          & \multicolumn{1}{l|}{86.56}          & \multicolumn{1}{l|}{99.55}          & 99.16          & \multicolumn{1}{l|}{392.11}          & \multicolumn{1}{l|}{2.05}           & \multicolumn{1}{l|}{398.64}          & \multicolumn{1}{l|}{2.47}            & \multicolumn{1}{l|}{407.78}          & 500.24            & \multicolumn{1}{l|}{1.29}          & \multicolumn{1}{l|}{0.06}          & \multicolumn{1}{l|}{1.92}          & \multicolumn{1}{l|}{0.38}          & \multicolumn{1}{l|}{1.83}           & 4.22             \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \textbf{\algoOnlinePQ} & \multicolumn{1}{l|}{\textbf{84.43}} & \multicolumn{1}{l|}{\textbf{79.47}} & \multicolumn{1}{l|}{\textbf{94.38}} & \multicolumn{1}{l|}{\textbf{99.39}} & \multicolumn{1}{l|}{\textbf{99.14}} & \textbf{99.15} & \multicolumn{1}{l|}{\textbf{1.35}}   & \multicolumn{1}{l|}{\textbf{0.96}}  & \multicolumn{1}{l|}{\textbf{3.17}}   & \multicolumn{1}{l|}{\textbf{382.15}} & \multicolumn{1}{l|}{\textbf{392.14}} & \textbf{19.03}    & \multicolumn{1}{l|}{\textbf{0.25}} & \multicolumn{1}{l|}{\textbf{0.25}} & \multicolumn{1}{l|}{\textbf{0.19}} & \multicolumn{1}{l|}{\textbf{2.33}} & \multicolumn{1}{l|}{\textbf{3.41}}  & \textbf{0.16}    \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{Navigation-based}} & \textbf{\algoHNSW}     & \multicolumn{1}{l|}{\textbf{99.97}} & \multicolumn{1}{l|}{\textbf{99.80}} & \multicolumn{1}{l|}{\textbf{99.96}} & \multicolumn{1}{l|}{\textbf{99.98}} & \multicolumn{1}{l|}{\textbf{88.94}} & \textbf{86.87} & \multicolumn{1}{l|}{\textbf{117.72}} & \multicolumn{1}{l|}{\textbf{15.83}} & \multicolumn{1}{l|}{\textbf{151.52}} & \multicolumn{1}{l|}{\textbf{584.60}} & \multicolumn{1}{l|}{\textbf{615.08}} & \textbf{11698.58} & \multicolumn{1}{l|}{\textbf{0.04}} & \multicolumn{1}{l|}{\textbf{0.03}} & \multicolumn{1}{l|}{\textbf{0.06}} & \multicolumn{1}{l|}{\textbf{0.11}} & \multicolumn{1}{l|}{\textbf{76.49}} & \textbf{1767.90} \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoNSW               & \multicolumn{1}{l|}{91.40}          & \multicolumn{1}{l|}{91.30}          & \multicolumn{1}{l|}{99.98}          & \multicolumn{1}{l|}{89.53}          & \multicolumn{1}{l|}{90.48}          & 88.04          & \multicolumn{1}{l|}{1721.73}         & \multicolumn{1}{l|}{212.89}         & \multicolumn{1}{l|}{454.59}          & \multicolumn{1}{l|}{689.47}          & \multicolumn{1}{l|}{1077.06}         & 6205.80           & \multicolumn{1}{l|}{161.95}        & \multicolumn{1}{l|}{20.28}         & \multicolumn{1}{l|}{0.09}          & \multicolumn{1}{l|}{80.61}         & \multicolumn{1}{l|}{113.37}         & 843.11           \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoNSG               & \multicolumn{1}{l|}{99.97}          & \multicolumn{1}{l|}{93.73}          & \multicolumn{1}{l|}{94.33}          & \multicolumn{1}{l|}{99.97}          & \multicolumn{1}{l|}{99.94}          & 94.80          & \multicolumn{1}{l|}{30.62}           & \multicolumn{1}{l|}{302.93}         & \multicolumn{1}{l|}{378.95}          & \multicolumn{1}{l|}{46.18}           & \multicolumn{1}{l|}{48.48}           & 1196.68           & \multicolumn{1}{l|}{0.01}          & \multicolumn{1}{l|}{20.26}         & \multicolumn{1}{l|}{22.80}         & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.03}           & 65.63            \\ \cline{2-20} 
\multicolumn{1}{|l|}{}                                  & \algoNNDecent          & \multicolumn{6}{l|}{N.A.}                                                                                                                                                                                    & \multicolumn{6}{l|}{N.A.}                                                                                                                                                                                         & \multicolumn{6}{l|}{N.A.}                                                                                                                                                                                  \\ \hline
\end{tabular}
}
\caption{
Break down the query latency into pending write latency and vector search latency. 
The pending write latency of \algoNNDecent exceeds 4 hours of wall time and triggers to terminate the whole \algoNNDecent evaluation. }
\label{tab:e2e_bd}
\end{table}

As discussed in Section\ref{subsec:general_setup}, we break down the query latency into two parts, i.e., \emph{pending writing latency} for the time spent in waiting for the pending writings and \emph{vector search latency} for the time spent in vector search after 
AKNN finishes its pending writing inside. The results are demonstrated in Table~\ref{tab:e2e_bd}. Due to the similar patterns, we use the inner product as an example. There are two major takeaways.
First, for most AKNN under most evaluated datasets, the pending writing latency is more dominant than vector search latency. For instance, it takes more than $75\%$ and $85\%$ of the total query latency in \algoOnlinePQ and \algoHNSW, respectively. Due to the large proportion and large amount, pending writing becomes the major performance bottleneck of querying. 
%
Second, the vector search latency of some AKNN is indeed lower than \algoBF in some datasets. For instance, \algoHNSW reduces $62\%$ vector search latency of \algoBF with reasonable recall (i.e., 0.61 in Table~\ref{tab:e2e_ip}) in \Msong dataset. Nevertheless, compared with static data case~\cite{li2019approximate}, this latency reduction is not guaranteed even under our evaluated datasets. When we shift the dataset into \DPR and \Trevi, \algoHNSW involves $271\times$ more and $1766\times$ more vector search latency than \algoBF.

%We can see that the latency of pending writings contributes to up to xxx. Nevertheless, this phenomenon never occurs under static data. Specifically, xxx.

\begin{quote}
    Observation \themyvar.
    It is helpful to improve recall and reduce vector search latency by queuing data and avoiding data dropping.
     However, this is not a practical useful option as it further increases the whole query latency.
\end{quote}
\stepcounter{myvar}
\begin{table}[]
 \resizebox{\textwidth}{!}{%
\begin{tabular}{|ll|llllll|llllll|llllll|llllll|llllll}
\cline{1-26}
\multicolumn{2}{|l|}{\multirow{2}{*}{Algorithms}}                                & \multicolumn{6}{l|}{Recall@10}                                                                                                                                                                         & \multicolumn{6}{l|}{Vector Search Latency ($\times 1000 ms$)}                                                                                                                                              & \multicolumn{6}{l|}{Pending Write Latency ($\times 1000 ms$)}                                                                                                                                                        & \multicolumn{6}{l|}{Query Latency ($\times 1000 ms$)}                                                                                                                                                                & \multicolumn{6}{l}{}                                                  \\ \cline{3-26}
\multicolumn{2}{|l|}{}                                                           & \multicolumn{1}{l|}{\Glove}        & \multicolumn{1}{l|}{\SIFT}         & \multicolumn{1}{l|}{\Msong}        & \multicolumn{1}{l|}{\Sun}          & \multicolumn{1}{l|}{\DPR}          & \Trevi        & \multicolumn{1}{l|}{\Glove}        & \multicolumn{1}{l|}{\SIFT}         & \multicolumn{1}{l|}{\Msong}        & \multicolumn{1}{l|}{\Sun}             & \multicolumn{1}{l|}{\DPR}          & \Trevi         & \multicolumn{1}{l|}{\Glove}          & \multicolumn{1}{l|}{\SIFT}           & \multicolumn{1}{l|}{\Msong}          & \multicolumn{1}{l|}{\Sun}             & \multicolumn{1}{l|}{\DPR}             & \Trevi          & \multicolumn{1}{l|}{\Glove}          & \multicolumn{1}{l|}{\SIFT}           & \multicolumn{1}{l|}{\Msong}          & \multicolumn{1}{l|}{\Sun}             & \multicolumn{1}{l|}{\DPR}             & \Trevi          &           &           &           &           &           &           \\ \cline{1-26}
\multicolumn{2}{|l|}{\textbf{\algoBF}}                                           & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \textbf{1.00} & \multicolumn{1}{l|}{\textbf{0.08}} & \multicolumn{1}{l|}{\textbf{0.08}} & \multicolumn{1}{l|}{\textbf{0.15}} & \multicolumn{1}{l|}{\textbf{0.16}}    & \multicolumn{1}{l|}{\textbf{0.24}} & \textbf{1.03}  & \multicolumn{1}{l|}{\textbf{0.35}}   & \multicolumn{1}{l|}{\textbf{0.35}}   & \multicolumn{1}{l|}{\textbf{0.44}}   & \multicolumn{1}{l|}{\textbf{0.54}}    & \multicolumn{1}{l|}{\textbf{0.50}}    & \textbf{1.50}   & \multicolumn{1}{l|}{\textbf{0.43}}   & \multicolumn{1}{l|}{\textbf{0.44}}   & \multicolumn{1}{l|}{\textbf{0.59}}   & \multicolumn{1}{l|}{\textbf{0.70}}    & \multicolumn{1}{l|}{\textbf{0.74}}    & \textbf{2.54}   & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \cline{1-26}
\multicolumn{1}{|l|}{\multirow{4}{*}{Ranging-based}}    & \textbf{\algoLSH}      & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.01}} & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.00}} & \multicolumn{1}{l|}{\textbf{0.00}} & \textbf{0.07} & \multicolumn{1}{l|}{\textbf{0.05}} & \multicolumn{1}{l|}{\textbf{0.03}} & \multicolumn{1}{l|}{\textbf{0.06}} & \multicolumn{1}{l|}{\textbf{0.29}}    & \multicolumn{1}{l|}{\textbf{0.02}} & \textbf{12.20} & \multicolumn{1}{l|}{\textbf{0.16}}   & \multicolumn{1}{l|}{\textbf{0.20}}   & \multicolumn{1}{l|}{\textbf{0.17}}   & \multicolumn{1}{l|}{\textbf{0.13}}    & \multicolumn{1}{l|}{\textbf{0.18}}    & \textbf{0.13}   & \multicolumn{1}{l|}{\textbf{0.21}}   & \multicolumn{1}{l|}{\textbf{0.23}}   & \multicolumn{1}{l|}{\textbf{0.23}}   & \multicolumn{1}{l|}{\textbf{0.42}}    & \multicolumn{1}{l|}{\textbf{0.20}}    & \textbf{12.33}  & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \algoPQ                & \multicolumn{1}{l|}{0.12}          & \multicolumn{1}{l|}{0.30}          & \multicolumn{1}{l|}{0.75}          & \multicolumn{1}{l|}{0.53}          & \multicolumn{1}{l|}{0.10}          & 0.53          & \multicolumn{1}{l|}{0.25}          & \multicolumn{1}{l|}{0.25}          & \multicolumn{1}{l|}{0.25}          & \multicolumn{1}{l|}{10.01}            & \multicolumn{1}{l|}{0.25}          & 0.26           & \multicolumn{1}{l|}{2.18}            & \multicolumn{1}{l|}{3.44}            & \multicolumn{1}{l|}{8.58}            & \multicolumn{1}{l|}{363.36}           & \multicolumn{1}{l|}{5.38}             & 21.87           & \multicolumn{1}{l|}{2.44}            & \multicolumn{1}{l|}{3.68}            & \multicolumn{1}{l|}{8.83}            & \multicolumn{1}{l|}{373.37}           & \multicolumn{1}{l|}{5.63}             & 22.14           &           &           &           &           &           &           \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \algoIVFPQ             & \multicolumn{1}{l|}{0.04}          & \multicolumn{1}{l|}{0.23}          & \multicolumn{1}{l|}{0.02}          & \multicolumn{1}{l|}{0.33}          & \multicolumn{1}{l|}{0.15}          & 0.42          & \multicolumn{1}{l|}{0.06}          & \multicolumn{1}{l|}{0.06}          & \multicolumn{1}{l|}{0.26}          & \multicolumn{1}{l|}{0.39}             & \multicolumn{1}{l|}{0.33}          & 1.99           & \multicolumn{1}{l|}{4.06}            & \multicolumn{1}{l|}{6.13}            & \multicolumn{1}{l|}{18.68}           & \multicolumn{1}{l|}{5.26}             & \multicolumn{1}{l|}{16.64}            & 20.24           & \multicolumn{1}{l|}{4.11}            & \multicolumn{1}{l|}{6.19}            & \multicolumn{1}{l|}{18.94}           & \multicolumn{1}{l|}{5.66}             & \multicolumn{1}{l|}{16.97}            & 22.22           &           &           &           &           &           &           \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \textbf{\algoOnlinePQ} & \multicolumn{1}{l|}{\textbf{0.12}} & \multicolumn{1}{l|}{\textbf{0.31}} & \multicolumn{1}{l|}{\textbf{0.82}} & \multicolumn{1}{l|}{\textbf{0.52}} & \multicolumn{1}{l|}{\textbf{0.10}} & \textbf{0.52} & \multicolumn{1}{l|}{\textbf{0.25}} & \multicolumn{1}{l|}{\textbf{0.25}} & \multicolumn{1}{l|}{\textbf{0.25}} & \multicolumn{1}{l|}{\textbf{17.04}}   & \multicolumn{1}{l|}{\textbf{0.25}} & \textbf{0.25}  & \multicolumn{1}{l|}{\textbf{2.28}}   & \multicolumn{1}{l|}{\textbf{0.96}}   & \multicolumn{1}{l|}{\textbf{16.61}}  & \multicolumn{1}{l|}{\textbf{382.01}}  & \multicolumn{1}{l|}{\textbf{29.57}}   & \textbf{161.91} & \multicolumn{1}{l|}{\textbf{2.53}}   & \multicolumn{1}{l|}{\textbf{1.21}}   & \multicolumn{1}{l|}{\textbf{16.86}}  & \multicolumn{1}{l|}{\textbf{399.04}}  & \multicolumn{1}{l|}{\textbf{29.81}}   & \textbf{162.16} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \cline{1-26}
\multicolumn{1}{|l|}{\multirow{4}{*}{Navigation-based}} & \textbf{\algoHNSW}     & \multicolumn{1}{l|}{\textbf{0.60}} & \multicolumn{1}{l|}{\textbf{0.90}} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{0.99}} & \multicolumn{1}{l|}{\textbf{0.80}} & \textbf{N.A.} & \multicolumn{1}{l|}{\textbf{0.04}} & \multicolumn{1}{l|}{\textbf{0.03}} & \multicolumn{1}{l|}{\textbf{0.05}} & \multicolumn{1}{l|}{\textbf{2362.95}} & \multicolumn{1}{l|}{\textbf{0.13}} & \textbf{N.A.}  & \multicolumn{1}{l|}{\textbf{733.51}} & \multicolumn{1}{l|}{\textbf{178.85}} & \multicolumn{1}{l|}{\textbf{560.26}} & \multicolumn{1}{l|}{\textbf{2048.23}} & \multicolumn{1}{l|}{\textbf{1008.00}} & \textbf{N.A.}   & \multicolumn{1}{l|}{\textbf{733.55}} & \multicolumn{1}{l|}{\textbf{178.88}} & \multicolumn{1}{l|}{\textbf{560.32}} & \multicolumn{1}{l|}{\textbf{4411.18}} & \multicolumn{1}{l|}{\textbf{1008.13}} & \textbf{N.A.}   & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \algoNSW               & \multicolumn{1}{l|}{0.14}          & \multicolumn{1}{l|}{0.55}          & \multicolumn{1}{l|}{0.34}          & \multicolumn{1}{l|}{0.78}          & \multicolumn{1}{l|}{0.52}          & N.A.          & \multicolumn{1}{l|}{0.08}          & \multicolumn{1}{l|}{0.10}          & \multicolumn{1}{l|}{0.09}          & \multicolumn{1}{l|}{662.16}           & \multicolumn{1}{l|}{0.32}          & N.A.           & \multicolumn{1}{l|}{1722.05}         & \multicolumn{1}{l|}{230.58}          & \multicolumn{1}{l|}{2659.85}         & \multicolumn{1}{l|}{727.73}           & \multicolumn{1}{l|}{1349.03}          & N.A.            & \multicolumn{1}{l|}{1722.13}         & \multicolumn{1}{l|}{230.68}          & \multicolumn{1}{l|}{2659.95}         & \multicolumn{1}{l|}{1389.90}          & \multicolumn{1}{l|}{1349.35}          & N.A.            &           &           &           &           &           &           \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \algoNSG               & \multicolumn{6}{l|}{N.A.}                                                                                                                                                                              & \multicolumn{6}{l|}{N.A.}                                                                                                                                                                                  & \multicolumn{6}{l|}{N.A.}                                                                                                                                                                                            & \multicolumn{6}{l|}{N.A.}                                                                                                                                                                                            &           &           &           &           &           &           \\ \cline{2-26}
\multicolumn{1}{|l|}{}                                  & \textbf{\algoNNDecent} & \multicolumn{6}{l|}{\textbf{N.A.}}                                                                                                                                                                     & \multicolumn{6}{l|}{\textbf{N.A.}}                                                                                                                                                                         & \multicolumn{6}{l|}{N.A.}                                                                                                                                                                                            & \multicolumn{6}{l|}{N.A.}                                                                                                                                                                                            &           &           &           &           &           &           \\ \cline{1-26}
\end{tabular}
}
\caption{Results of cross-validation. N.A. means that the evaluation of certain algorithms and certain datasets exceeds 4h wall time, and therefore unable to get further results. We observe that all of the N.A. is caused by the large overhead of pending writtings.}
\label{tab:e2e_cross}
\end{table}


To further investigate the hidden reasons for our surprising observation, we conduct another group of evaluations for cross-validation. We kept all the settings the same as Tables~\ref{tab:e2e_ip} and ~\ref{tab:e2e_bd}, except the data source waits for AKNN to make sure all of the data is fully ingested. 
Specifically, this is achieved by using sufficiently large in-memory queues. The results are summarized in Table~\ref {tab:e2e_cross}. There are three major take-aways. First, by comparing the recall reported in Table~\ref{tab:e2e_cross} with Table~\ref{tab:e2e_ip}, we observe that avoiding the data dropping increases the recall for most AKNN. For instance, if there is no data dropping for \algoHNSW to ingest \Msong online, recall is improved from $0.61$ to $1.00$. This is as expected, and there are more relevant vectors ingested by AKNN to answer the query if we guarantee the completeness of ingested data. 
%
Second, by comparing Table~\ref{tab:e2e_cross} with Table~\ref{tab:e2e_bd}, we also find that guaranteeing the completeness of ingested data is also helpful in reducing vector search latency. In this way, more 
AKNN outperform \algoBF in searching vectors and it aligns better with the common beliefs in conducting on static data~\cite{li2019approximate}.
For instance, the vector search latency of \algoOnlinePQ in \DPR is largely reduced from $3.43s$ to $0.25s$, as it spends less time in traversing distant vectors when complete data collection is ingested. 
%
Lastly, if we go back to the end-to-end query latency shown in  Table~\ref{tab:e2e_cross} v.s. that in Table~\ref{tab:e2e_ip}, there are no practical useful improvements but only the enlarged total latency, e.g., from about $691s$ to $1008s$ for \algoHNSW to ingest \DPR.
This is because most AKNN is intrinsically slower to be updated than the data source, and maintaining their consistent and complete view of data itself is a costly process, such as memory copies and its resulting cache missing. This kind of overhead is first absorbed in the pending writings, then increases the whole latency of the query.


%In this way, the comparison of vector search latency and recall looks similar to prior works like~\cite{li2019approximate}, and some AKNN like \algoHNSW do outperform brutal force way in vector search latency. Nevertheless, the synchronization overhead between the data source and AKNN further increases pending writing latency, thereby the overall query latency.


%\xianzhi{--Table of breakdown proportion and absolute value}
%Even if we only focus on the vector search latency, we observe that most AKNN fail to outperform the brutal force baseline. In particular, \algoHNSW, which is considered to be one of the optimal AKNN in static data, leads to xxx more vector search latency.
%As discussed in Section~\ref{}, if one AKNN fail to catch up with the data source's rate of feeding data, it has to drop data. When the query asks about this part of dropped data, AKNN like \algoHNSW spend a lot of time to reaching the candidate results, often much longer than expected. To further validate this, we conduct another group of evaluations as summarized in Table~\ref{}.
%We kept all the settings the same as Table~\ref{}, except the data source waits for AKNN to make sure all of the data is fully ingested. Specifically, the data source synchronizes with AKNN with sufficiently large in-memory queues.
%In this way, the comparison of vector search latency and recall looks similar to prior works like~\cite{li2019approximate}, and some AKNN like \algoHNSW do outperform brutal force way in vector search latency. Nevertheless, the synchronization overhead between the data source and AKNN further increases pending writing latency, thereby the overall query latency.


==> Experiment.tex <==

\section{Evaluate}


\label{sec:methodology}
In the following section, we first introduce experimental configurations and then present the results. 
%\newcounter{myvar}
%\setcounter{myvar}{1}
% We refer interested readers to Appendix~\ref{appendix} for more information on the evaluation protocols and implementations.
% Please add the following required packages to your document preamble:
% \usepackage{multirow}




\textbf{Distance Measure.} 
We consider both L2 distance~\cite{li2019approximate} and inner product distance~\cite{aguerrebere2024locally} to define the vector similarities, and inner product distance is our default if not otherwise specified. 
%

\begin{table}[t]
\centering
    \centering
    \resizebox{0.7\textwidth}{!}{%
   \begin{tabular}{|l|l|l|l|}
\hline
\multirow{7}{*}{Real-world} & \textbf{Name}                                                   & \textbf{Description} & \textbf{Dimension} \\ \cline{2-4} 
                            & \Glove~\cite{li2019approximate}                                 & Text embedding       & $100$              \\ \cline{2-4} 
                            & \SIFT~\cite{li2019approximate}                                  & Image                & $128$              \\ \cline{2-4} 
                            & \Msong~\cite{li2019approximate}                                 & Audio                & $4208$             \\ \cline{2-4} 
                            & \Sun~\cite{li2019approximate}                                   & Image                & $512$              \\ \cline{2-4} 
                            & \DPR~\cite{aguerrebere2024locally}                              & Text embedding       & $768$              \\ \cline{2-4} 
                            & \Trevi~\cite{li2019approximate}                                 & Image                & $4096$             \\ \hline
\multirow{2}{*}{Synthetic}  & \Random~\cite{Pytorch}                                          & i.i.d values         & Adjustable         \\ \cline{2-4} 
                            & \Wte~\cite{aguerrebere2024locally,warthunderWiki,loper2002nltk} & Text embedding       & $768$              \\ \hline
\end{tabular}
}
\caption{Datasets.}
\label{tab:realworld_workloads}
\end{table}


\textbf{Datasets.} 
Following the methodologies outlined in ~\cite{li2019approximate,aguerrebere2024locally}, we encompass a wide variety of \emph{real-world workloads} as detailed in Table~\ref{tab:realworld_workloads}, which span across several application domains, including text embeddings (\DPR) and image processing (\Trevi). The \DPR dataset was reconstructed using the source code and corpus provided by ~\cite{aguerrebere2024locally}, whereas the remaining datasets were obtained from ~\cite{li2019approximate}. As a preliminary step, we normalize each dataset using the \emph{torch::norm} function to ensure that the values range between -1 and 1.

In addition to these real-world datasets, we introduce two \emph{synthetic workloads}: \Random and \Wte. The \Random dataset consists of values generated by the \emph{torch::random} function, which produces a sequence of independent and identically distributed (i.i.d.) uniform values between $0$ and $1$. This approach allows for the configuration of dimensions and volumes of vectors to suit various needs. The \Wte dataset is designed to mimic the text embedding process of \DPR, but with input text sentences generated synthetically. 
Specifically, we make up simple sentences with three words for subject, predicate and object, respectively, and then utilize the encoder to generate embeddings. Both subject and object are nouns, and we can introduce controlled nature data distribution shifts as discussed in ~\cite{aguerrebere2024locally} by changing the category scope of choosing nouns, such as USSR land vehicles against USA aircrafts from the video game Warthunder~\cite{warthunderWiki}. On the contrary, the predicate part is just a random verb from NLTK~\cite{loper2002nltk} without any biased or shifted distribution.
Notably, the machine learning models to generate embeddings are kept static, with no fine-tuning or continual learning applied. The default size for \Wte is set at 768 dimensions with 100K rows.
%To create this dataset, we first selected a category of nouns—specifically, names of weapons from the video game Warthunder~\cite{warthunderWiki}—and combined these with 100 verbs randomly chosen from the nltk package ~\cite{loper2002nltk} to form sentences. Each sentence in the dataset follows the structure <noun 1> <verb> <noun 2>.'' with a corresponding query What <verb> <noun 2>?'' By varying the noun categories, such as comparing USSR land vehicles against USA aircrafts, we introduce controlled nature data distribution shifts as discussed in ~\cite{aguerrebere2024locally}. Notably, the machine learning models to generate embeddings are kept static, with no fine-tuning or continual learning applied. The default size for \Wte is set at 768 dimensions with 100K rows.

\textbf{AKNN Implementation.} We unify the implementation of the examined AKNN algorithms into one C++ codebase, using static compilation to guarantee consistency across experiments. We use the IEEE 754 32-bit floating-point (FP32) format for representing vector elements and \emph{torch::Tensor} to represent the vectors, such that our benchmark is fully compatible with LibTorch and PyTorch without extra conversions. While certain AKNN algorithms might benefit from algorithm-specific or distance-metric-specific optimizations, e.g., learning to hash~\cite{li2023learning}, learning to route~\cite{baranchuk2019learning}, randomized distance comparison~\cite{gao2023high} and Locally-Adaptive Quantization ~\cite{aguerrebere2024locally}, 
The AKNN optimizations, such as~\cite{li2023learning,baranchuk2019learning,gao2023high,aguerrebere2024locally}, are
excluded in this Section~\ref{sec:methodology} for a fair comparison, and we separately review AKNN optimizations in Section~\ref{}. 
 We focus on in-memory AKNN, and leave out-of-memory case~\cite{yue2023optimizing} or disk-memory corporation~\cite{alafate2019faster,singh2021freshdiskann} for future works. 
\xianzhi{Not that, we didn't intentionally tune or optimize any algorithm to solely maximized recall or merely minimized query latency. Instead, we follow the recommended default settings from existing works such as ~\cite{gionis1999similarity,jegou2010product,muja2014scalable,xu2018online,malkov2014approximate,li2019approximate,fu2019fast}. These settings are found to achieve a practically useful balance between accuracy and query efficiency, as validated in ~\cite{li2019approximate}. }




 \textbf{Deployment.}
Our evaluation primarily unfolds on a xxx processor, with AKNN seamlessly adapting to parallel and distributed computing through a straightforward sharding approach~\cite{wang2021milvus}. Algorithm-specific parallelization, such as concurrent write of vertices in \algoHNSW~\cite{singh2021freshdiskann,aguerrebere2024locally}, is excluded due to the complexity of a fair alignment.
This directs our focus towards single-threaded evaluation. 
 
\newcounter{customstep}
\setcounter{customstep}{0}
\renewcommand{\thecustomstep}{\textbf{Step \arabic{customstep}}}

\newenvironment{customitemize}{
  \begin{list}{\thecustomstep}{%
    \usecounter{customstep}%
    \setlength{\labelwidth}{4em}%
    \setlength{\leftmargin}{\labelwidth}%
    \addtolength{\leftmargin}{\labelsep}%
    \itemsep 0pt%
  }%
}{
  \end{list}
}
 
\input{Evaluations/Overall}
\input{Evaluations/Environ}
\input{Evaluations/Other}


==> OnlineSettings.tex <==
\section{From Static Data to Online Ingestion}
In this section, we discuss the major differences in moving from static data to online ingestion in evaluating AKNN algorithms, followed by algorithm-specific adaptions involved.
\subsection{General Configuration and Performance Metrics}
\label{subsec:general_setup}
Rather than the common configurations in ~\cite{li2019approximate,gionis1999similarity,jegou2010product,muja2014scalable,xu2018online,malkov2014approximate,li2019approximate,fu2019fast}, which load AKNN with all data 
in its offline stage and never change the data storage of AKNN, we are concerned about 
\emph{What if the data ingested online?}
By default, we initially load AKNN with 50K rows of vector in its offline stage, the overhead of this stage is excluded in our measure. Afterwards, we enter the online ingestion phase by feeding AKNN with new data (by default 4K rows/second). The micro batches~\cite{huang2019gpipe,yuan2022decentralized} are utilized to agglomerate data at the AKNN's side, with each sized 4K rows by default. When there is no longer new data from the source, we immediately submit a search query of multiple vectors to the AKNN. 

We are concerned about two common performance metrics, i.e., \emph{query recall} and \emph{query latency}. As discussed in Section~\ref{sec:bg}, \emph{query recall} is an accuracy metric, and it measures the fraction of the true nearest neighbours that are correctly identified by the algorithm out of all possible true nearest neighbours. By default, we report the {query recall} of searching for $10$ similar vectors for each one of the $100$ inputs, or \emph{ 100 recall@10} for short.
\emph{Query latency}, on the other hand, is an efficiency metric to measure the time from a query's submission to the time when AKNN returns the results. 

Although we utilize the same performance metrics as existing works like ~\cite{li2019approximate}, there are two major differences introduced by online ingestion to be noted. First, the data source will be regardless of AKNN's capacity but keep feeding data at the assigned steady speed. In this way, AKNN has to drop data as discussed in Section~\ref{sec:intro}, which worsens \emph{Query recall} and potentially also increases  \emph{Query latency}. Second, the AKNN may still be conducting some ongoing writing when a query is submitted, and the pending writing for data ingestion blocks vector search in this case, thereby contributing to the large \emph{Query latency}. 

\subsection{Adapting AKNN Algorithms to Online Ingestion}
Most AKNN are mainly intended for static data, and we summarize how they are adapted to online ingestion in this part.


\textbf{To Adapt AKNN with Minor Changes.} We observe that some of the AKNN inherently build their index in an incremental and one-pass manner, without any repeated scan or reference on the yet-to-come data, specifically, \algoLSH, \algoNSW and \algoHNSW. Moreover, \algoOnlinePQ is intentionally designed for ingesting new data online. These algorithms require no significant changes to be adapted in the online ingestion case, and we just align their API and I/O data structure in our evaluation codebase.

\textbf{To Adapt AKNN with Enforced Assumptions.} 
\algoPQ, \algoIVFPQ, and xx also ingest data in an incremental and one-pass manner. Nevertheless, this process additionally relies on an established knowledge of data distributions. 
The knowledge-building process requires multiple scans on full data collection and involves notoriously large overhead, e.g., xxx for \algoIVFPQ over xxx data scale. Therefore, 
we set up the knowledge for them only at the offline stage and assume it is still valid in online ingestion. As discussed before, any overhead in the offline stage is excluded from our evaluation.

\textbf{To Adapt AKNN with Algorithm Modifications.} 
The rest of the evaluated AKNN, i.e., \algoNNDecent,  \algoDPG and \algoNSG are highly specialized for static data, specifically, xxxxx. To adapt them into online ingestion case, we xxxx.
\xianzhi{
---
write your own analysis and optimizations here
@zhuoyan @xinjing 
} 
\algoNSG (Navigable Spreading-out Graph) depends on a pre-built graph by brute force. A navigation point would be selected randomly as the entry point for subsequent insertion and search. For the rest of the points, all neighbor candidates would be searched and linked starting from the navigation point so that all sub-graphs are connected with the navigation point. To adapt \algoNSG into online ingestion case, the ingested points would go through a similar process as those from the pre-built graph, that they carry out a global neighbor search from the navigation point and update the graph structure accordingly.


%\subsection{Challenges of Distribution Shifts}


==> Opts.tex <==
\section{Revisit AKNN Optimizations in Online Ingestion}
%There are various AKNN optimization techniques~\cite{li2023learning,NIPS2008_d58072be,baranchuk2019learning,aguerrebere2024locally,gao2023high} as discussed in Section~\ref{sec:methodology}. Despite each of them being specially designed for certain AKNN algorithms or certain distance metrics, we observe that they strategically fall into two orthogonal categories: i.e., machine-learning-based AKNN~\cite{li2023learning,NIPS2008_d58072be,baranchuk2019learning} and optimized distance computation~\cite{baranchuk2019learning,aguerrebere2024locally}.
There are two categories of AKNN optimizations as discussed in Section~\ref{sec:bg}, i.e., machine-learning-based AKNN~\cite{li2023learning,NIPS2008_d58072be,baranchuk2019learning} and optimized distance computation~\cite{baranchuk2019learning,aguerrebere2024locally}.
We evaluate each of them in the following.
\subsection{Machine-Learning-Based AKNN}

\begin{table}[]
\resizebox{0.99\textwidth}{!}{%
\begin{tabular}{|l|llll|llll|}
\hline
\multirow{2}{*}{Algoroithms} & \multicolumn{4}{l|}{Steady Distrition}                                                                                                   & \multicolumn{4}{l|}{Distribution Shift}                                                                                                  \\ \cline{2-9} 
                             & \multicolumn{1}{l|}{Recall@10} & \multicolumn{1}{l|}{Query Latency} & \multicolumn{1}{l|}{Vector Search Latency} & Pending Write Latency & \multicolumn{1}{l|}{Recall@10} & \multicolumn{1}{l|}{Query Latency} & \multicolumn{1}{l|}{Vector Search Latency} & Pending Write Latency \\ \hline
\algoBF                      & \multicolumn{1}{l|}{1.000}     & \multicolumn{1}{l|}{0.19}          & \multicolumn{1}{l|}{0.12}                  & 0.07                  & \multicolumn{1}{l|}{1.000}     & \multicolumn{1}{l|}{0.21}          & \multicolumn{1}{l|}{0.14}                  & 0.07                  \\ \hline
\algoLSH w/o ML              & \multicolumn{1}{l|}{0.003}     & \multicolumn{1}{l|}{0.03}          & \multicolumn{1}{l|}{0.01}                  & 0.03                  & \multicolumn{1}{l|}{0.003}     & \multicolumn{1}{l|}{0.04}          & \multicolumn{1}{l|}{0.01}                  & 0.03                  \\ \hline
\algoLSH w/ ML               & \multicolumn{1}{l|}{0.024}     & \multicolumn{1}{l|}{0.10}          & \multicolumn{1}{l|}{0.10}                  & 0.01                  & \multicolumn{1}{l|}{0.374}     & \multicolumn{1}{l|}{5.82}          & \multicolumn{1}{l|}{5.82}                  & 0.01                  \\ \hline
\end{tabular}
}
\caption{Optimizing AKNN by machine learning, the example AKNN is \algoLSH and the example datasets are \DPR (for steady distribution case) and \Wte (for distribution shift case), the unit of latency is $\times 1000ms$. We follow all of the settings in Table~\ref{tab:e2e_ip}, \xianzhi{and the distribution shift starts at the same time when online ingestion begins}. The neural network in machine learning is pre-trained, and it conducts inference on the CPU in our evaluation.}
%\caption{Optimizing AKNN by machine learning, the example dataset is \DPR, and we follow all of the default settings in Table~\ref{}, the unit of latency is $\times 1000ms$}
\label{tab:opt_aknn_ml}
\end{table}



We select the \algoLSH as the example to study the impact of using matching learning, \algoLSH is the only AKNN to catch up with fast data source (up to $4K rows/s$) in our previous evaluations (Section~\ref{subsec:overall}), but it constantly suffers from low accuracy in real-world datasets. For a fair comparison, we optimize \algoLSH by replacing its random projection hash function with a pre-trained MLP, while keeping other data structures and workflows the same.
The MLP is trained by following the spectral hashing loss function as detailed in ~\cite{NIPS2008_d58072be}. We acknowledge that more complicated structures are also applicable such as using transforms~\cite{li2023learning}, and we leave them for future works due to their additional complexity related to incorporating new hardware like GPUs.
%
As detailed in Table~\ref{tab:opt_aknn_ml}, using machine learning significantly improves the accuracy by at least $ 7\times$.
The query latency and vector search latency are increased when using machine learning, and they are mostly caused by the static overhead of using neural networks. However, they are still attractive compared with \algoBF, i.e., $45\%$ less query latency.  
Furthermore, we observe that machine learning reduces the pending writing latency of AKNN (i.e., $66\%$ less compared with raw \algoLSH), as it
leads to a more accurate assignment of interested vectors.

%\xianzhi{We next select \algoHNSW for investigation. Contrary to \algoLSH, \algoHNSW is the most accurate AKNN but always suffers from the high overhead of updating the graph. We optimize \algoHNSW by following~\cite{li2023learning}, where the routing heuristics of \algoHNSW is replaced by xxx and others remain unchanged.The result in xx also confirms the superiority of optimizing AKNN by machine learning.}


Nevertheless, how to handle the distribution shifts is still an opening challenge for machine learning itself, and the suboptimal performance of learning leads to a significant performance downgrade of AKNN. 
Although the recall seems to be even better, i.e., $0.374$ in this case, the query latency is extremely high. This is because the AKNN can not find the straight-forward matches under ML-based \algoLSH during the distribution shift, therefore, it downgrades into an exhaustive traverse on all of the buckets, which is even more costly than \algoBF.
We envision more advanced techniques such as online continual learning~\cite{li2022camel} to solve this problem, as well as solving other related implementation issues like re-encoding the existing buckets~\cite{xu2018online}. 
\subsection{Optimized Distance Computation in AKNN}
\xianzhi{We choose \algoHNSW as the illustration example, we follow ~\cite{gao2023high} and ~\cite{} for the approximate computing under Inner Product and L2 distance metrics, respectively, and we follow ~\cite{aguerrebere2024locally} to conduct the data compression of vectors.}

xxxxx


==> RelatedWork.tex <==
\section{Related Work}
\label{appendix:related}
 AKNN algorithms have evolved significantly since first proposed in 1998~\cite{indyk1998approximate}. Early developments focused on optimizing search efficiency and accuracy through various techniques such as locality-sensitive hashing (LSH)~\cite{gionis1999similarity}, tree-based indexing~\cite{weber1998quantitative}, and graph-based methods~\cite{malkov2018efficient}, primarily for static datasets. In contrast, recent advancements have targeted the adaptation of AKNN algorithms for dynamic environments, where data continually evolves. Notable contributions include Xu et al.’s incremental clustering~\cite{xu2018online,xu2022proximity}, which dynamically adjusts data structures with new information, and the work by Aguerrebere et al.~\cite{aguerrebere2024locally} and Singh et al.~\cite{singh2021freshdiskann}, which explore vector compression and SSD-aware optimizations to accommodate incremental vector additions. Despite these innovative approaches, there remains a distinct lack of comprehensive benchmarks in practically reflecting dynamic data ingestion. 
%that accurately reflect the continuous evolution of datasets in practical settings. 
%highlighting a critical research gap that recent studies seek to address.

% \section{Related Work}
% \label{appendix:related}
% AKNN algorithms have been extensively studied for their efficiency in handling static datasets. Seminal works by Indyk and Motwani~\cite{indyk1998approximate} introduced the concept of approximate nearest neighbor search, laying the groundwork for numerous subsequent studies. Techniques such as locality-sensitive hashing (LSH)~\cite{gionis1999similarity}, tree-based indexing~\cite{weber1998quantitative}, and graph-based approaches~\cite{malkov2018efficient} have evolved, each aiming to balance search accuracy with computational efficiency. However, these approaches primarily address scenarios where the dataset does not change over time.
% Recognizing the limitations of traditional AKNN algorithms in dynamic environments, recent research has focused on extending these methods for online data ingestion. Xu et al.~\cite{xu2018online,xu2022proximity} introduce incremental clustering that dynamically adjusts the data structure as new information arrives. 
% Aguerrebere et al.~\cite{aguerrebere2024locally} and Singh et al.~\cite{singh2021freshdiskann} explore
% vector compression and SSD-aware optimizations in proxy graphs, respectively,  to accommodate the incremental addition of vectors.
% These efforts mark significant progress in adapting AKNN algorithms to more realistic, evolving data streams.
% Despite their efficiency across applications such as computer vision and natural language processing tasks~\cite{li2019approximate}, the evaluation of AKNN algorithms often overlooks the dynamic nature of real-world data. Typically assumed to operate on static vector collections, these evaluations do not reflect the continuous evolution of datasets in practical settings~\cite{aguerrebere2024locally,singh2021freshdiskann}. 
% Recent studies have begun to adapt specific AKNN algorithms towards dynamic workloads~\cite{aguerrebere2024locally,singh2021freshdiskann,xu2022proximity}. Despite these efforts, a comprehensive benchmark for AKNN that that accurately mirror real-world data dynamics is still lacking.

